Convex Optimization for Parameter Synthesis in MDPs

Probabilistic model checking aims to prove whether a Markov decision process (MDP) satisfies a temporal logic specification. The underlying methods rely on an often unrealistic assumption that the MDP is precisely known. Consequently, parametric MDPs (pMDPs) extend MDPs with transition probabilities that are functions over unspecified parameters. The parameter synthesis problem is to compute an instantiation of these unspecified parameters such that the resulting MDP satisfies the temporal logic specification. We formulate the parameter synthesis problem as a quadratically constrained quadratic program (QCQP), which is nonconvex and is NP-hard to solve in general. We develop two approaches that iteratively obtain locally optimal solutions. The first approach exploits the so-called convex-concave procedure (CCP), and the second approach utilizes a sequential convex programming (SCP) method. The techniques improve the runtime and scalability by multiple orders of magnitude compared to black-box CCP and SCP by merging ideas from convex optimization and probabilistic model checking. We demonstrate the approaches on a satellite collision avoidance problem with hundreds of thousands of states and tens of thousands of parameters and their scalability on a wide range of commonly used benchmarks.

==> applications.tex <==
\section{Case Studies}\label{sec:applications}

\subsection{Distributed Processes: CSMA/CA}

\subsection{Randomisation in Movement Planning: Robot control}



==> approximation.tex <==
\section{Sequential Geometric Programming}\label{sec:approximation}

We showed how to efficiently obtain a feasible solution
% of the parameter and scheduler variables 
 for Problem~\ref{prob:pmdpsyn} by solving GP~\eqref{eq:min_rand_geofull}--\eqref{eq:rewcomputation_geofull}. %In some applications, finding a feasible solution for a pMDP synthesis problem itself is useful. 
%In some applications, this is itself a useful result which enables the solution of problems involving thousands of states and parameters. %
%The ability to efficiently obtain such a feasible solution is useful by itself. %, due to the good scaling with respect to the number of parameters in the pMDP. 
%In particular, the good scaling with the number of parameters in $V$ cannot be understated. (For example, existing parameter synthesis tools can only handle thousands of states with tens of parameters. With the GP~\eqref{eq:min_rand_geofull}--\eqref{eq:rewcomputation_geofull}, we can handle thousands of states with thousands of parameters.)
%However, we are further interested in obtaining optimal solutions to Problem~\ref{prob:pmdpsyn}. In general, an SGP cannot be solved for the optimal solution efficiently. Moreover, the GP~\eqref{eq:min_rand_geofull}--\eqref{eq:rewcomputation_geofull} obtained by convexifying the SGP cannot be used to compute an optimal solution.
%Solving an SGP to obtain the global optimal solution is not efficient in general, however we can 
%However, an optimal solution to the GP~\eqref{eq:min_rand_geofull}--\eqref{eq:rewcomputation_geofull} does not necessarily optimize the original objective $f$ in Problem~\ref{prob:pmdpsyn}. 
%While the general SGP cannot be efficiently solved, we can still do well with respect to the original objective $f$. 
%
%However, this solution does not necessarily optimize the original objective $f$ in Problem~\ref{prob:pmdpsyn}. 
We propose a \emph{sequential convex programming} trust-region method to compute a local optimum of the SGP~\eqref{eq:min_rand}--\eqref{eq:rewcomputation}, following~\cite[\S{}9.1]{boyd2007tutorial}, solving a sequence of GPs. We obtain each GP by replacing signomial functions in equality constraints of the SGP~\eqref{eq:min_rand}--\eqref{eq:rewcomputation} with \emph{monomial approximations} of the functions. 



%The local optimum of the SGP provides a local optimal solution to Problem~\ref{prob:pmdpsyn}. Note that in some applications, a feasible solution to Problem~\ref{prob:pmdpsyn} is itself useful.
%
%In this section we observe that our original problem actually forms  a \emph{signomial program} (SGP), for which one can compute \emph{locally optimal solutions} efficiently~\cite{boyd2007tutorial}. 
%
%
%\subsection{Signomial programming}
%
%We identify a subclass of NLPs called \emph{signomial programs} and explain certain useful properties. Then we show how by a simple insight the NLP \eqref{eq:min_rand}--~\eqref{eq:well-defined_probs_rand} is transformed to such a program.
%Note: This explanation is written for Case A and C. As the objective for Case B involves minimizing the probability, it is tricky to find a local maximum point for this case.
%We return to the SGP~\eqref{eq:min_rand}--\eqref{eq:rewcomputation}. To find a locally optimal solution, we compute the best local monomial approximation for each non-monomial equality constraint. We enforce the approximation over a trust region. We then replace each non-monomial equality constraint with its monomial approximation, and solve a local trust-region GP.
%The monomial approximations are defined using a valuation of the variables of the SGP, and the approximation is only valid for valuations which belong to a region known as the trust-region. We describe the process of 
%
%
%The solution of each geometric program in the sequence is used to obtain a feasible solution to the SGP, which in turn is used to obtain the next geometric program in the sequence. The sequence of solutions of the geometric programs so obtained yields a sequence of feasible solutions to Problem~\ref{prob:pmdpsyn}, and the latter sequence converges to a locally optimal solution of Problem~\ref{prob:pmdpsyn}.
%
%
%that in turn yield a sequence of decreasing values of the objective $f$ in \eqref{eq:min_rand}. The solution sequence will eventually converge to a locally optimal solution of Problem~\ref{prob:pmdpsyn}. 
%Each successive member of the sequence, obtained by solving a geometric program, yields a feasible solution to Problem~\ref{prob:pmdpsyn} with a smaller value of the objective $f$ in \eqref{eq:min_rand}. 
%A valuation of the SGP variables Solving the geometric program 
%The monomial approximations are defined using a valuation of the variables of the SGP, and the approximation is only valid for valuations which belong to a region known as the trust-region. Each valuation obtained as a solution to the GP serves as  
%
\begin{definition}[Monomial approximation]
Given a posynomial $f \in \posys[\Var]$, variables $\Var = \{x_1,\dots,x_n\}$, and a valuation $u \in \valuations^\Var$, a \emph{monomial approximation $\hat f\in\monos[\Var]$ for $f$ near $u$} is 
\begin{align*}
	\forall i. 1 \leq i \leq n
	\quad
	\hat f = f[u]
	\prod_{i=1}^{n}\Bigg(\dfrac{x_{i}}{u(x_i)}\Bigg)^{a_{i}},
	\quad
	\text{where }
	a_{i}=\dfrac{u(x_i)}{f[u]}\dfrac{\partial f}{\partial x_{i}}[u].
\end{align*}	
\end{definition}
Intuitively, we compute a \emph{linearization} $\hat f$ of $f\in\posys[\Var]$ around a fixed valuation $u$.
%
%
%\paragraph{Trust region.}
We enforce the fidelity of monomial approximation $\hat{f}$ of $f \in \posys[\Var]$ by restricting valuations to remain within a set known as \emph{trust region}. We define the following constraints on the variables $\Var$ with $t > 1$ determining the size of the trust region:
\begin{align}
	\label{eq:trust_region}
	\forall i. 1 \leq i \leq n
	\quad (\nicefrac{1}{t})\cdot u(x_i) \leq x_i \leq t\cdot u(x_i)
\end{align}
% 
%
%
%%Generally, we want $t$ to have a value of the form $1 + \epsilon$, where $0 < \epsilon \ll 1$, to make sure that the error of
%%the approximation is small.
%%$f(w_{s})$ is the best local monomial approximation of $\sum_{s'\in S}P(s,s')$ in state $s$ and $n$ is the number of variables. 
%
%
%
For a given valuation $u$, we approximate the SGP~\eqref{eq:min_rand}--\eqref{eq:rewcomputation} to obtain a \emph{local GP} as follows. %First, we replace the objective function of the SGP by its monomial approximation near $u$.
First, we apply a \emph{lifting} procedure (Section~\ref{sec:lifting}) to the SGP ensuring that all constraints consist of posynomial functions. The thus obtained posynomial inequality constraints are included in the local GP.
After replacing posynomials in every equality constraint by their monomial approximations near $u$, the resulting monomial equality constraints are also included.
Finally, we add trust region constraints~\eqref{eq:trust_region} for scheduler and parameter variables. The objective function is the same as for the SGP.
The optimal solution of the local GP is not necessarily a feasible solution to the SGP. 
Therefore, we first normalize the scheduler and parameter values to obtain well-defined probability distributions. These normalized values are used to compute precise probabilities and expected cost using \tool{PRISM}. The steps above provide a feasible solution of the SGP.

We use such approximations to obtain a sequence of feasible solutions to the SGP approaching a local optimum of the SGP. 
First, we compute a feasible solution $u^{(0)}$ for Problem~\ref{prob:pmdpsyn} (Section \ref{sec:geometric}), 
%These values form a feasible solution $u^{(0)}$ to SGP~\eqref{eq:min_rand}--\eqref{eq:rewcomputation} which is the 
%
forming the initial point of a sequence of solutions $u^{(0)},\ldots, u^{(N)}, N \in \N$. 
The solution $u^{(k)}$ for $0\leq k\leq N$ is obtained from a local GP defined using $u^{(k-1)}$ as explained above.

%Using solution $u^{(k)}, we obtain a local GP by locally approximating SGP~\eqref{eq:min_rand}--\eqref{eq:rewcomputation} near $u^{(k)}$. 

%The optimal solution of this GP does not necessarily yield a feasible solution to the SGP. 
%We normalize the scheduler and parameter values for the optimal solution to obtain well-defined probability distributions. These normalized values are then used to compute reachability probabilities and expected cost values as was done for $u^{(1)}$. In this way, we obtain $u^{(k+1)}$ ( which is a feasible solution of SGP~\eqref{eq:min_rand}--\eqref{eq:rewcomputation}) from $w^{(k)}$. %
%Once gain, \tool{PRISM} is used to obtain $u^{(k+1)}$ from $w^{(k)}$.

The parameter $t$ for each iteration $k$ is determined based on its value for the previous iteration, and the ratio of $ f\left[u^{(k-1)}\right] $ to $f\left[u^{(k-2)}\right]$, where $f$ is the objective function in \eqref{eq:min_rand}. The iterations are stopped when $\left| f\left[u^{(k)}\right] - f\left[u^{(k-1)}\right] \right| <  \epsilon$. Intuitively, $\epsilon$ defines the required improvement on the objective value for each iteration; once there is not enough improvement the process terminates.
%%The trust region must get smaller with the iteration count $k$, because otherwise there is no guarantee that the local method will converge without oscillations. In practice, any rule for which $t\to 1^+$ as $k\to\infty$ will work. We define $t$ at iteration $k$ as $t = 1 + 1 / k$. 
%When $?$ holds, the sequential optimization is ended and $?$ is taken as the locally optimal solution. 
%\hp{Formal statement that the sequence reaches a locally optimal solution.}

%As we will see in the next section, this local method allows us to improve the objective value from the initial valuation and scheduler by a factor of $100$ or more.
%\ip{check this number}
%We denote the valuation of the variables $\Var$ obtained as a feasible valuation  of the SGP~\eqref{eq:min_rand}--\eqref{eq:rewcomputation} at iteration $k$ by $u^{(k)} \in \valuations^\Var$. The valuation $u^{(k)}$ contains scheduler variable assignments $(\sigma^{s,\act})^{(k)}$, transition probabilities $\probmdp(s,\act,s')^{(k)}$, reachability probabilities $p_s^{(k)}$, and costs $c_s^{(k)}$. \hp{The valuation should contain a `sub-valuation' of the variables \dots}

%We locally approximate the SGP~\eqref{eq:min_rand}--\eqref{eq:rewcomputation} near a valuation $u^{(k)}$ at iteration $k$ to obtain a trust-region GP denoted by $\text{GP}(k)$ over the variables $\Var$. The procedure to obtain $\text{GP}(k)$ consists of replacing every equality constraint of the SGP~\eqref{eq:min_rand}--\eqref{eq:rewcomputation} by its monomial approximation around $u^{(k)}$. The objective function of the SGP is also replaced by its monomial approximation near $u^{(k)}$. %With this approximation in place, the SGP~\eqref{eq:min_rand}--\eqref{eq:rewcomputation} becomes $\text{GP}(k)$. 
%We solve $\text{GP}(k)$ to obtain a valuation denoted by $w^{(k)}$.
%Note that the trust-region GPs obtained here are different from the GP~\eqref{eq:min_rand_geofull}--\eqref{eq:rewcomputation_geofull}. The trust-region GPs provide (a sequence of) local solutions to the SGP~\eqref{eq:min_rand}--\eqref{eq:rewcomputation} which converge to a locally optimal solution of Problem~\ref{prob:pmdpsyn}. In contrast, GP~\eqref{eq:min_rand_geofull}--\eqref{eq:rewcomputation_geofull} provides feasible solutions to Problem~\ref{prob:pmdpsyn}.% In fact, the main use of GP~\eqref{eq:min_rand_geofull}--\eqref{eq:rewcomputation_geofull} is to provide an initial point for the sequence 

% \paragraph{Sequential convex optimization.}
% We then repeat the process.
% The trust region must get smaller with the iteration count $k$, because
% otherwise there is no guarantee that the local method will converge without
% oscillations. In practice, any rule for which $t\to 1^+$ as $k\to\infty$ will
% work. 
% 
% As we will see in the next section, this local method allows us to
% improve the objective value from the initial valuation and scheduler by a
% factor of $100$ or more.
% \ip{check this number}


%for the posynomial term in Equation~\ref{eq:well-defined_probs} near the initial guess $x(k)$ with following, where $x(k)$ is the vector that has the variable assignments from initial guess for previous iteration:

%After computing $f(w)$, we solve the following problem:
%\begin{align}
%	\text{maximize } &\quad p_{\sinit}\\
%	\text{such that}\\
%%		 &\quad p_{\sinit}\leq \lambda\label{eq:strategyah:lambda}\\
%	\forall s\in T.	 &\quad p_s=1\\
%	\forall s\in S\setminus T.	&\quad p_s = \sum_{s'\in S}	P(s,s')\cdot p_{s'}\\
%	\forall s\in S.	 &\quad f(w_{s})=1\\
%	&\quad (1/k)x(k)_{i}\leq x_{i} \leq kx(k)_{i}, i=1,2,...,n
%\end{align}
%		

% \begin{tabbing}
%     \rule{\linewidth}{0.4pt}\\
%     \textbf{algorithm:} sequential convex programming\\
%     \textbf{given}: pMPD Problem~\ref{prob:pmdpsyn} \\
%     \textbf{output}: better valuation $u$ and scheduler $\sched$.\\
%     \textbf{begin} \\
%         \quad
% 		\= 1. \= Solve GP~\eqref{eq:min_rand_geofull}--\eqref{eq:rewcomputation_geofull}
% 				to obtain initial valuation and scheduler\\
% 		\> 2. set $k:=0$\\
%         \> 3. \> \textbf{repeat}\\
%         \> \> \quad \= approximate around
% 			$((\sigma^{s,\act})^{(k)}, \probmdp(s,\act,s')^{(k)}, p_s^{(k)}, c_s^{(k)})$\\
% 		\> \> \> solve $\text{GP}(k)$\\
% 		\> \> \> perform updates\\
%         \> \> \textbf{until} convergence criterion\\
%     \textbf{end}\\
%     \rule{\linewidth}{0.4pt}
% \end{tabbing}


%As this problem is a GP, we could solve this problem efficiently and the solution of this problem would be taken for the next iteration and we repeat this procedure until convergence to a local maximum. The procedure would be similar in Case C, as we would compute the local momomial approximation of the posynomials in Equations~\ref{eq:welldefined_sched_rand} and \ref{eq:well-defined_probs_rand}. Then, we would iteratively compute the next guess until we converge to a local maximum.
%


==> convex.tex <==
\chapter{Convex Solvers for Feasibility}[Iteratively solving convex over-approximations]
\label{chap:encoding}
\newcommand{\qcqpmatrix}{Q}

\paragraph{Summary}
Feasibility in pMCs and pMDPs is an ETR-hard problem, giving little hope for a scalable and general solution. 
However, as guessing one valuation right suffices to solve the problem, there is plenty of room for heuristics.
This chapter develops such a heuristic by employing convex optimisation. 
First, we formulate the ETR formula as a \emph{quadratically-constrained quadratic program} (QCQP). 
To allow for efficient solving techniques, 
we massage the QCQP formulation into a \emph{difference-of-convex} (DC) problem.
The \emph{convex-concave procedure} (CCP) yields local optima of a DC problem by a convexification towards a convex quadratic program, 
amenable for state-of-the-art solvers such as \Gurobi~\cite{gurobi}.
Yet, black-box CCP solvers suffer from severe numerical issues and only solve small problems.
Therefore, in the final part, we integrate the procedure with probabilistic model checking, creating a method that
yields (1)~a speedup of multiple orders of magnitude compared to just using CCP as a black box and (2)~ensures the correctness of the solution. %as shown by the experiments at the end of the chapter.

\paragraph{Origins}
This chapter resembles \cite{DBLP:conf/atva/CubuktepeJJKT18} with some extensions and clarifications.


\paragraph{Background}
The chapter builds on top of the ETR-encoding for feasibility in pMDPs under demonic nondeterminism from~\cref{sec:etrencodingreachability}. 
For convenience, the encoding is repeated at the start of the chapter. 
The notation is in line with the ETR encoding, which means that some notation is slightly unusual from an optimisation perspective.


\section{QCQP Reformulation of Feasibility Synthesis}
\index{feasibility!using convex optimisation}

Within this chapter, we consider the following problem:
Given an affine pMDP $\pmdp = (S, \init, \Act, \pars, \pprob)$ with target states $\target$, a threshold $\lambda$, an $\varepsilon > 0$,  and a property $\varphi \coloneq \probop{\leq \lambda}{\target}$, find an $\varepsilon$-preserving valuation $\val \in \accept[\pmdp]{\forall,\varphi}$, i.e., find $\val$ such that $\instantiated{\pmdp}{\val} \mdpmodels{\forall} \varphi$. An $\varepsilon$-preserving valuation assigns to every transition at least $\varepsilon$, see \cref{def:epspreserving}. For conciseness, we assume that $\pprob(s,\act,s') \in \QQ$ implies $ \pprob(s,\act,s') \geq \varepsilon$.
Furthermore, as convention $n \coloneq |S|$ and $k \coloneq |\pars|$.
%\begin{remark}
The method in this chapter is also applicable to expected rewards or lower bounds, with adaptions that we have seen for the ETR encodings in \cref{sec:parametric:etr}. We restrict ourselves to only one case for conciseness.
%\end{remark}



\paragraph{Recap of the encoding}
We start with the ETR encoding for demonic feasibility on pMDPs, as discussed in \vref{constr:ubreachdnondet}.
% which generalises the linear program from the Bellman inequations for parameter-free MDPs, cf.\ \cref{sec:models:mdplps}. 
A satisfying assignment to these constraints yields a
valuation in $\accept[\pmdp]{\forall,\varphi}$.
As we are only interested in $\varepsilon$-preserving valuations, the constraints in \cref{constr:ubreachdnondet} may be simplified by ideas from \cref{sec:parametric:etr}. Together with the constraints for $\varepsilon$-preserving valuations we obtain:
%In \cref{constr:ubreachgpdnondet} we give this simplification together with the constraints for $\varepsilon$-preserving valuations:
\begin{constraints}
Let $\pmdp$ be a pMDP, $\varphi \coloneq \probop{\leq \lambda}{\target}$ a property, and some graph-preservation constant $\varepsilon \in \RRpos$. 
We consider the following constraint system with real-valued variables $\{ p_s \mid s \in S_{>0} \coloneq S \setminus \pzeroexstates[\target]{\mathrm{gp}} \}$ and variables for each parameter:
\label{constr:ubreachgpdnondet}
\begin{align*}
    & p_\init \cleq \lambda, \\
	& \pprob(s,\act,s') \cgeq \varepsilon & & \text{for all }s, s' \in S, \act \in \EnAct(s),  \\
	& \sum_{s' \in S} \pprob(s,\act,s') \ceq 1 & & \text{for all }s \in S, \act \in \EnAct(s), \\
	& p_s \ceq 1 & & \text{for all } s \in \target, \\
	%& p_s \ceq 0 & & \text{for all } s \in \pzeroexstates[\target]{\mathrm{gp}} \\
	&  p_s \cgeq \sum_{s' \in S_{>0}} \pprob(s,\act, s') \cdot p_{s'} & &\text{for all } s \in  S_{>0} \setminus  \target , \act \in \EnAct(s). 
	\end{align*}%	
	Variables $p_s$ thus encode that the probability from state $s$ to the target is at least $p_s$.
	The constraints encode that the probability from state $p_\init$ is at most $\lambda$, that all transitions have probability at least $\varepsilon$,  that the outgoing transitions are a well-defined distribution over successor states, and encode the Bellman characterisation lifted to pMDPs. 
\end{constraints}
The constraints also include a minor optimisation that allows for a concise notation below: No variables for the reachability from zero-states are added to the constraints.
 Instead, these variables are immediately substituted with zero. This substitution is reflected by summing over the non zero-state successors in the last constraint.

\begin{figure}
\centering
	\tikzsetnextfilename{qcqp_runningex}
	\input{figures/qcqp_runningex}
	\caption{Example pMC}
	\label{fig:qcqp:runningex}
\end{figure}
\begin{example}
	We use the pMC in \cref{fig:qcqp:runningex} to illustrate the transformation of the encoding presented in this chapter.\label{ex:qcqp:runningexintro}
	We keep $\lambda$ as a constant, use $p_i$ to denote $p_{s_i}$, and obtain the constraints:
\[%	\begin{align*}
		p_0 \cleq \lambda , \;\;\; \varepsilon \cleq x \cleq 1 - \varepsilon , \;\;\; p_3 \ceq 1, \;\;
		p_0 \cgeq x \cdot p_1  , \;\;\; p_1 \cgeq  (1-x)\cdot p_2 , \;\;\; p_2 \cgeq x \cdot p_3.
\]%	\end{align*}
\end{example}


\paragraph{QCQPs}
In affine pMDPs all  entries of $\pprob$ are linear and thus all constraints in \cref{constr:ubreachgpdnondet} are quadratic.
We rewrite the ETR formula as a standard form of a \emph{quadratically-constrained quadratic program} (\keyword{QCQP})~\cite{BV04}.
In general, a QCQP is an optimisation problem with a quadratic objective function and $m$ quadratic constraints, written in standard form:  
%
\begin{constraints}[QCQP standard form]
\label{constr:standardqcqp}
\begin{align*}
&  \text{minimise}   \quad \vec{v}^T A_0 \vec{v} + b_0^T \vec{v}+c_0\quad \text{such that} \\
&   \vec{v}^T A_i \vec{v} + b_i^T \vec{v}+c_i \cleq 0 \quad\text{for all } i \in \{1,\ldots,m\} ,
\end{align*}
where $\vec{v}$ is a vector of $l$ \emph{variables} and the coefficients are $A_i \in \RR^{l \times l}$, $b_i \in \RR^l$, $c_i \in \RR$ for $0\leq i\leq m$. 
We assume $A_0,\ldots, A_m$ are symmetric without loss of generality.

\end{constraints}
Equality-constraints of the form $\vec{v}^T A_i \vec{v} + b_i^T \vec{v}+c_i = 0$ may be encoded by
\[ 
	 \vec{v}^T A_i \vec{v} + b_i^T \vec{v}+c_i \leq 0\text{ and }-\vec{v}^T A_i \vec{v} - b_i^T \vec{v} - c_i \leq 0\ .
\]


If $A_i=0$ for all $0 \leq i \leq m$, the polynomials $b_i^T \vec{v}+c_i$ are \emph{linear}, and the QCQP is in fact an LP.
If every $A_i$ is positive semi-definite (PSD), the function $\vec{v}^T A_i \vec{v} + q_i^T \vec{v}+r_i$ is \emph{convex},  the QCQP is a \emph{convex optimisation problem}, and may be solved in polynomial time~\cite{DBLP:journals/mp/AlizadehG03}.
If any $A_i$ is not PSD, the resulting QCQP is nonconvex. Checking whether a quadratic constraint system is satisfiable is ETR-complete~\cite{Schaefer2013}, cf.\ \cref{thm:etr:bquad}.



\paragraph{Reformulating feasibility as QCQP}
To ease the presentation, we deviate from the standard ETR encoding and move closer to an optimisation formulation.
\begin{constraints}
\label{constr:feasibilityqcqp}
 The following constraints are a reformulation of \cref{constr:ubreachgpdnondet} to the standard QCQP form (for the quadratic constraints) in \cref{constr:standardqcqp}\footnote{We allow an affine non-zero right-hand side (rhs) for better readability. Naturally, the rhs may be set to zero by subtracting the rhs from the left-hand side (lhs). Furthermore, we have flipped lhs and rhs, as this notation is closer to the standard presentation of the equation system (and easier to read).}:
	\begin{align*}
	&	\text{minimise} \quad p_\init 
			\quad\text{such that} \\
							&  p_{\init}\cleq \lambda,\\
 &  p_s\ceq1\quad & & \text{for all }s \in T,\\
			 & \pprob(s,\act,s')\cgeq \varepsilon\quad  & & \text{for all } s,s'\in S, \act\in\EnAct(s),	\\
				 & \sum_{s'\in S}\pprob(s,\act,s')\ceq1 \quad & & \text{for all } s\in S, \act\in\EnAct(s), \\
			& p_s \cgeq \vec{v}^{T}\qcqpmatrix_{s,\act} \vec{v}+q_{s,\act}^T\vec{v},  & & \text{for all } s\in S_{>0} \setminus  \target, \act\in \EnAct(s), 
		\end{align*}
where $\vec{v}$ is a vector consisting of the probability variables $p_s$ for all $s\in S$ and the pMDP parameters, i.e., $\vec{v}$ has $n+k$ rows. 
Furthermore, $\qcqpmatrix_{s,\act}\in\RR^{(n+k)\times(n+k)}$ is a symmetric  matrix and $q_{s,\act}\in\RR^{(n+k)}$.
\end{constraints}
\begin{example}
	\label{ex:qcqp_transformation}
	
We reformulate the ETR encoding in \cref{ex:qcqp:runningexintro}.
	We omit matrix columns and matrix rows that only contain zeros to have a concise representation. Accordingly, the vectors are pruned.
	\begin{align*}
			&\text{minimise}\quad p_\init \quad
			\text{such that} \\
			&\lambda \cgeq p_{0} ,  1-\varepsilon  \cgeq x \cgeq \varepsilon, \quad p_{3}\ceq 1, \\
			&  p_0 \cgeq \begin{bmatrix}
    x \\
    p_{1}
\end{bmatrix}^T \qcqpmatrix_{0} \begin{bmatrix}
    x \\
    p_{1}
\end{bmatrix},\quad
 p_{1} \cgeq   \begin{bmatrix}
    x \\
    p_{2}
\end{bmatrix}^T \qcqpmatrix_{1} \begin{bmatrix}
    x \\
    p_{2}
\end{bmatrix} +p_{2} ,\quad
 p_{2} \cgeq 
\begin{bmatrix}
    x \\
    p_{3}
\end{bmatrix}^T \qcqpmatrix_{2} \begin{bmatrix}
    x \\
    p_{3}
\end{bmatrix}, 
					\end{align*}	

\[ \text{ with}\quad \qcqpmatrix_0 \coloneq \begin{bmatrix}
    0       & \nicefrac{1}{2} \\
     \nicefrac{1}{2}      & 0
\end{bmatrix},\quad 
\qcqpmatrix_1 \coloneq \begin{bmatrix}
    0       & - \nicefrac{1}{2} \\
   - \nicefrac{1}{2}     & 0
\end{bmatrix},\quad
\qcqpmatrix_2 \coloneq \begin{bmatrix}
    0       & \nicefrac{1}{2} \\
     \nicefrac{1}{2}      & 0
\end{bmatrix}.
  \]
  Equivalently, but denoted more precisely, the quadratic constraints are:
  \begin{align*}
 &  	\begin{bmatrix}
    x \\
    p_{1}
\end{bmatrix}^T \qcqpmatrix_{0} \begin{bmatrix}
    x \\
    p_{1}
\end{bmatrix} + \begin{bmatrix} 1 \end{bmatrix}^T \begin{bmatrix} p_0 \end{bmatrix}  \cleq 0,  \\
&  \begin{bmatrix}
    x \\
    p_{2}
\end{bmatrix}^T \qcqpmatrix_{1} \begin{bmatrix}
    x \\
    p_{2}
\end{bmatrix} + \begin{bmatrix} -1 \\ 1 \end{bmatrix}^T \begin{bmatrix} p_1 \\ p_{2}\end{bmatrix} \cleq  0, \\
& 
\begin{bmatrix}
    x \\
    p_{3}
\end{bmatrix}^T \qcqpmatrix_{2} \begin{bmatrix}
    x \\
    p_{3}
\end{bmatrix} + \begin{bmatrix} 1 \end{bmatrix}^T \begin{bmatrix} p_2 \end{bmatrix}  \cleq 0. 
  \end{align*}
   We want to stress that $\qcqpmatrix_0 \neq \qcqpmatrix_2$, as the rows and columns that are zero (and not displayed here) are different.
\end{example}
%\paragraph{Construction of the QCQP}
In the example above, we magically constructed the right matrices. Below we clarify the (trivial) construction.
We use matrices $\qcqpmatrix_{s,\act}$ to capture the \emph{quadratic} part and the vector $q_{s,\act}$ to capture the \emph{affine} part of the constraints.

More precisely, consider an affine transition probability $a \cdot x + b \coloneq \pprob(s,\act,s')$ with $a,b\in\RR$.
The polynomial occurs in the constraint from \cref{constr:ubreachgpdnondet} in $\pprob(s,\act,s') \cdot p_{s'}$.
% = (a\cdot x+b)\cdot p_{s'}$.
The quadratic part thus occurs as $a\cdot x\cdot p_{s'}$ and the affine part as $b \cdot p_{s'}$.

We focus on 
the product $\vec{v}^T\qcqpmatrix_{s,\act}\vec{v}$, which denotes the sum over all products of entries in $\vec{v}$.
Thus, in $\qcqpmatrix_{s,\act}$, each row or column corresponds either to a probability variable $p_s$ for a state $s\in S$ or to a parameter $v \in V$. 
Thus, the matrix cells indexed $(x, p_{s'})$ and $(p_{s'}, x)$ correspond to the product of parameter $x$ with the state-variable $p_{s'}$.
As the matrix $\qcqpmatrix_{s,\act}$ needs to be symmetric, there are two entries in $\qcqpmatrix_{s,\act}$ that represent the product of $p_s$ and $x$.
These two entries are summed in $\vec{v}^T\qcqpmatrix_{s,\act}\vec{v}$.
Thus, the coefficient $a$ is represented by $\nicefrac{a}{2}$ in both entries, making $\qcqpmatrix_{s,\act}$  a symmetric matrix.
For example, if $\pprob(s,\act,s')=\nicefrac{1}{5} \cdot x+\nicefrac{1}{3}$, we insert $\nicefrac{1}{10}$ in $\qcqpmatrix_{s,\act}$ at the two entries for $x \cdot p_{s'}$.
Similarly, we construct $q_{s,\act}$ by setting the entry for $p_{s'}$ to $b$.
We do not modify the affine functions for the QCQP form.
%

\noindent
The following observation is not surprising, as the feasibility problem is ETR-hard.
\begin{proposition}
	The QCQP in~\cref{constr:feasibilityqcqp} is nonconvex in general.
\end{proposition}
\begin{proof}
The matrices $\qcqpmatrix_{0}, \qcqpmatrix_{1}, \qcqpmatrix_{2}$ in \cref{ex:qcqp_transformation} have an eigenvalue of ${-}\nicefrac{1}{2}$ and are not PSD.
Thus, the constraints and the resulting QCQP are nonconvex. 
\end{proof}


\section{Efficiently Solving the QCQP}
\label{sec:ccp}
The QCQP in \cref{constr:feasibilityqcqp} is nonconvex and hard to solve in general.
We provide a solution by employing a heuristic called the \emph{convex-concave procedure} (\keyword{CCP})~\cite{lipp2016variations}, which relies on the ability to efficiently solve convex optimisation problems.
Later in  this section, we improve this method by employing probabilistic model checking.

\subsection{A CCP approach to the feasibility problem}
\paragraph{Overview}
Roughly, the CCP approach for the feasibility problem is captured by \cref{fig:ccploop}. It is a search for a solution of the  nonconvex QCQP, that literately solves approximations of the QCQP in form of convex DC problems around some initial $\hat{v} \in \RR^{l}$. 
For any satisfying valuation of such a DC problem,
we may check some penalty-value of this solution. If this penalty is zero, we have found a solution to the original nonconvex QCQP. 
Otherwise, we update (or guess) a new $\vec{v}$ which we use to convexify the QCQP. This loop may get stuck, which requires restarts. 
\begin{figure}
	\centering
	\tikzsetnextfilename{qcqp_naiveloop}
	\input{figures/qcqpnaiveloop}
	\caption{Penalty CCP loop}
	\label{fig:ccploop}
\end{figure}
We start with the construction of the (penalty-)DP,
then discuss the update function, and finally discuss how to tune this method by an improved method for generating the DP. We also include some remarks on how we selected the numerous constants in the method.


\paragraph{DC reformulation}
The CCP computes a \emph{local optimum} of a nonconvex \emph{difference-of-convex} (\keyword{DC}) problem. 
\begin{constraints}[DC standard form with polynomial constraints]
\label{constr:dcstandardform}
	\begin{align*}
			&\text{minimise } \quad f_0-g_0 \quad\text{such that} \nonumber \\
							 & f_i-g_i\cleq 0 \quad\text{for all  }1\leq i \leq m,
		\end{align*}

with convex $f_i, g_i \in \QQ[\vec{v}]$ for $0\leq i \leq m$. 
\end{constraints}
The polynomials ${-}g_i$ are \emph{concave}.	 
Every quadratic polynomial can be rewritten as a DC polynomial,
i.e., as difference of two convex polynomials.
Consider the quadratic polynomial $\vec{v}^{T}\qcqpmatrix_{s,\act} \vec{v}+q_{s,\act}^T\vec{v}$ from~\cref{constr:feasibilityqcqp}.
We decompose the matrix $\qcqpmatrix_{s,\act}$ into the difference of two matrices
%
\begin{align}
	\qcqpmatrix_{s,\act} = \qcqpmatrix^+_{s,\act} - \qcqpmatrix^-_{s,\act}\quad\text{with }\quad \qcqpmatrix^+_{s,\act} \coloneq \qcqpmatrix_{s,\act}+tI \text{ and } \qcqpmatrix^-_{s,\act} \coloneq tI, 
	\label{eq:makepsd}
\end{align}
%
where $I$ is the identity matrix and $t \in \RRpos$ is sufficiently large to render $\qcqpmatrix^+_{s,\act}$ PSD, i.e., larger than the largest eigenvalue of $\qcqpmatrix_{s,\act}$. 
Then, we rewrite \[ \vec{v}^{T}\qcqpmatrix_{s,\act} \vec{v}+q_{s,\act}^T\vec{v} \cleq 0 \rightsquigarrow \underbrace{\vec{v}^{T}\qcqpmatrix^+_{s,\act}\vec{v}+q_{s,\act}^T\vec{v}}_{f_i} - \underbrace{\vec{v}^{T}\qcqpmatrix^-_{s,\act} \vec{v}}_{g_i} \cleq 0,\] which is in the form of~\cref{constr:dcstandardform}.
Together, we obtain the following constraints:
\begin{constraints}[DC for feasibility]
\label{constr:qcqp:dc} The following constraints are a reformulation of \cref{constr:ubreachgpdnondet} to the standard DC form  in \cref{constr:dcstandardform}:
	\begin{align*}
	&	\text{minimise} \quad p_\init
			\quad\text{such that} \\
							& p_{\init}\cleq \lambda,\\
 & p_s\ceq1\quad & & \text{for all }s \in T,\\
			 & \pprob(s,\act,s')\cgeq \varepsilon\quad  & & \text{for all} s,s'\in S, \act\in\EnAct(s),	\\
				 & \sum_{s'\in S}\pprob(s,\act,s')\ceq1 \quad & & \text{for all } s\in S, \act\in\EnAct(s), \\
			&p_s \cgeq \vec{v}^{T}\qcqpmatrix^{+}_{s,\act} \vec{v}+q_{s,\act}^T\vec{v} - \vec{v}^{T}\qcqpmatrix^{-}_{s,\act} \vec{v}  & & \text{for all } s\in S_{>0}\setminus T, \act\in \EnAct(s). 
		\end{align*}
\end{constraints}
The reformulations so far are equivalences, formalised by the following corollary.
\begin{corollary}
\label{cor:qcqp:dcreformulation}
	The solutions for \cref{constr:ubreachgpdnondet} and \cref{constr:qcqp:dc} coincide.
\end{corollary}


\begin{example}
Recall the pMC in \cref{fig:qcqp:runningex} and the QCQP from \cref{ex:qcqp_transformation}.  All matrices $\qcqpmatrix_s$ in the QCQP are not PSD.
	\label{ex:dc}
We construct a DC problem with $t=1$ for all $\qcqpmatrix_s$:
%
\begin{align*}
			&\text{minimise } \quad p_{0} \quad \text{such that}\\
			&\lambda \cgeq p_{0}, \quad 1-\varepsilon  \cgeq x \cgeq \varepsilon,\quad p_{3}\ceq 1, \\
			& p_0 \cgeq \begin{bmatrix}
    x \\
    p_{1}
\end{bmatrix}^T \begin{bmatrix}
    1       & \nicefrac{1}{2} \\
    \nicefrac{1}{2}       & 1
\end{bmatrix} \begin{bmatrix}
    x \\
    p_{1}
\end{bmatrix} - \begin{bmatrix}
    x \\
    p_{1}
\end{bmatrix}^T \begin{bmatrix}
    1       & 0 \\
    0       & 1
\end{bmatrix} \begin{bmatrix}
    x \\
    p_{1}
\end{bmatrix}, \\
& p_{1} \cgeq \begin{bmatrix}
    x \\
    p_{2}
\end{bmatrix}^T \begin{bmatrix}
    1       & {-}\nicefrac{1}{2} \\
    {-}\nicefrac{1}{2}       & 1
\end{bmatrix} \begin{bmatrix}
    x \\
    p_{2}
\end{bmatrix} - \begin{bmatrix}
    x \\
    p_{2}
\end{bmatrix}^T \begin{bmatrix}
    1       & 0 \\
    0       & 1
\end{bmatrix} \begin{bmatrix}
    x \\
    p_{2}
\end{bmatrix} +p_{2},\\
& p_{2} \cgeq  \begin{bmatrix}
    x \\
    p_{3}
\end{bmatrix}^T \begin{bmatrix}
    1       & \nicefrac{1}{2} \\
    \nicefrac{1}{2}       & 1
\end{bmatrix} \begin{bmatrix}
    x \\
    p_{3}
\end{bmatrix} - \begin{bmatrix}
    x \\
    p_{3}
\end{bmatrix}^T \begin{bmatrix}
    1       & 0 \\
    0       & 1
\end{bmatrix} \begin{bmatrix}
    x \\
    p_{3}
\end{bmatrix}. 
		\end{align*}
\end{example}


\paragraph{Penalty CCP for DP}
For the obtained DC problem, we consider the iterative \emph{penalty CCP method}~\cite{lipp2016variations}.
The procedure is initialised with any initial assignment $\hat{v}$ for the variables $v \in \vec{v}$.
In the \emph{convexification} stage, we compute affine approximations in form of a linearisation of $g_{i}$ around $\hat{v}$:
	\begin{align}
	\tilde{g}_i \coloneq g_i[\hat{v}]+\nabla g_i[\hat{v}]^{T}\cdot(\vec{v}-\hat{v}),
	\label{eq:linearisations}
		\end{align}	
where $\nabla g_i$ is the gradient of the polynomial $g_i$ at $\hat{v}$.
The polynomial  $f_i-\tilde{g}_i$ is clearly convex. 
The gradient of $\vec{v}^T\qcqpmatrix^-_{s,\act}\vec{v}$ is $2 \cdot \qcqpmatrix^-_{s,\act}\hat{v}$. 
\begin{constraints}[Over-approximating DC for feasibility]
\label{constr:qcqp:overapproxdc}
For a pMDP and property as before and some valuation $\hat{v}$ for \emph{all} variables in the DC, consider the following optimisation problem:
	\begin{align*}
	&	\text{minimise} \quad p_\init 
			\quad\text{such that} \\
							& p_{\init}\cleq \lambda,\\
 &  p_s\ceq1\quad & & \text{for all }s \in T,\\
			 & \pprob(s,\act,s')\cgeq \varepsilon\quad  & & \text{for all } s,s'\in S, \act\in\EnAct(s),	\\
				 & \sum_{s'\in S}\pprob(s,\act,s')\ceq1 \quad & & \text{for all } s\in S, \act\in\EnAct(s), \\
			& p_s \cgeq \vec{v}^{T}\qcqpmatrix^{+}_{s,\act} \vec{v}+q_{s,\act}^T\vec{v} - \hat{v}^{T}\qcqpmatrix^{-}_{s,\act}(2\vec{v} - \hat{v})  & & \text{for all } s\in S_{>0}\setminus T, \act\in \EnAct(s). 
		\end{align*}
\end{constraints}
The following proposition clarifies the meaning of the over-approximation:
\begin{proposition}
\label{prop:qcqp:overapprox}
A satisfying assignment for \cref{constr:qcqp:overapproxdc}  is also satisfying \cref{constr:qcqp:dc}.	
\end{proposition}
\begin{proofsketch}
Using the notation of \cref{constr:dcstandardform} and equation \eqref{eq:linearisations}:
It holds that: \[ f_i - g_i \leq f_i - \tilde{g_i}. \]
This inequality is the direct consequence of the following standard result on convex functions\footnote{Readers unfamiliar with this result may want to  draw the derivative of a univariate convex function.}:
Let $f \in \QQ[\vars]$ be convex. For $\val, \val' \in \Val$, 
\[ f[\val'] \geq f[\val] + \nabla f[\val](\val' - \val).\]
We thus obtain $g_i \geq \tilde{g_i}$ for all $1 \leq i \leq m$, and consequently ${-}g_i \leq {-}\tilde{g_i}$.
Then, $f_i - g_i \leq f_i - \tilde{g_i}$.
From that result, it is clear that any $\val$ that satisfies 
\[ p_s \cgeq \vec{v}^{T}\qcqpmatrix^{+}_{s,\act} \vec{v}+q_{s,\act}^T\vec{v} - \tilde{v}^{T}\qcqpmatrix^{-}_{s,\act}(2\vec{v} - \tilde{v}) \]
also satisfies
 \[ p_s \cgeq \vec{v}^{T}\qcqpmatrix^{+}_{s,\act} \vec{v}+q_{s,\act}^T\vec{v} - \vec{v}^{T}\qcqpmatrix^{-}_{s,\act}\vec{v}.  \]
 The claim follows, as all other constraints remain untouched.
\end{proofsketch}

The stricter set of constraints is often too strict and may not have any feasible solution.
To loosen the constraints, a \emph{penalty variable} $\delta_{s,\act}$ for all $s\in S \setminus T$ and $\act\in\Act$ is added to all convexified constraints.
These variables allow us to measure the `amount' of infeasibility.
The larger the assigned value for a penalty variable, the larger the violation.
We then seek to minimise the violation of the original DC constraints by minimising the sum of the penalty variables.
%If this sum is minimized to $0$, we have a feasible solution to the convexified problem. 
The resulting convex optimisation problem is:
\begin{constraints}[penalty-DC for feasibility]
\label{constr:qcqp:final}
For an approximating DC over variables as in \cref{constr:qcqp:overapproxdc}, a constant penalty constant $\tau \in \RRpos$, and additional \emph{penalty variables} $\{ \delta_{s,\act} \mid s \in S, \act\in \EnAct(s)\}$ we formulate the following constraint system:
	\begin{align*}
	&	\text{minimise} \quad p_\init + \tau \cdot \sum_{s}\sum_{\act} \delta_{s,\act}
			\quad\text{such that} \\
							& p_{\init}\cleq \lambda,\\
 &  p_s\ceq1\quad & & \text{for all }s \in T,\\
  & \delta_{s,\act} \cgeq 0 & & \text{for all }s \in S, \act \in \EnAct(s), \\
			 & \pprob(s,\act,s')\cgeq \varepsilon\quad  & & \text{for all } s,s'\in S, \act\in\EnAct(s),	\\
				 & \sum_{s'\in S}\pprob(s,\act,s')\ceq1 \quad & & \text{for all } s\in S, \act\in\EnAct(s), \\
			& p_s + \delta_{s,\act} \cgeq \vec{v}^{T}\qcqpmatrix^{+}_{s,\act} \vec{v}+q_{s,\act}^T\vec{v} - \hat{v}^{T}\qcqpmatrix^{-}_{s,\act}(2\vec{v} - \hat{v})  & & \text{for all } s\in S_{>0}\setminus T, \act\in \EnAct(s). 		
		\end{align*}
		
\end{constraints}
\begin{example}
We continue with \cref{ex:dc} and bring the constraints into the form of \cref{constr:qcqp:final}. We assume some valuation $\hat{v}$ for each  $v \in \{ x, p_0, p_1, p_2, p_3 \}$.
	\begin{align*}
		&	\text{minimise } \quad p_{0}+\tau\sum_{i=0}^2 \delta_{i} \quad \text{such that}  \nonumber\\
			&\lambda \cgeq p_{0} , \quad 1-\varepsilon  \cgeq x \cgeq \varepsilon , \quad p_{3}\ceq 1 \\
			& \delta_{0}+p_{0} \cgeq \begin{bmatrix}
    x \\
    p_{1}
\end{bmatrix}^T \begin{bmatrix}
    1       & \nicefrac{1}{2} \\
    \nicefrac{1}{2}       & 1
\end{bmatrix} \begin{bmatrix}
    x \\
    p_{1}
\end{bmatrix} - \begin{bmatrix}
    \hat{x} \\
    \hat{p_1}
\end{bmatrix}^T \begin{bmatrix}
    1       & 0 \\
    0       & 1
\end{bmatrix} \begin{bmatrix}
    2\cdot x-\hat{x} \\
    2\cdot p_{1}-\hat{p_1}
\end{bmatrix}, \\
&\delta_{1}+p_{1} \cgeq \begin{bmatrix}
    x \\
    p_{1}
\end{bmatrix}^T \begin{bmatrix}
    1       & {-}\nicefrac{1}{2} \\
    {-}\nicefrac{1}{2}       & 1
\end{bmatrix} \begin{bmatrix}
    x \\
    p_{2}
\end{bmatrix} - \begin{bmatrix}
    \hat{x} \\
    \hat{p_2}
\end{bmatrix}^T \begin{bmatrix}
    1       & 0 \\
    0       & 1
\end{bmatrix} \begin{bmatrix}
    2\cdot x-\hat{x} \\
    2\cdot p_{2}-\hat{p_2}
\end{bmatrix} +p_{2}, \\
& \delta_{2}+p_{2} \cgeq \begin{bmatrix}
    x \\
    p_{3}
\end{bmatrix}^T \begin{bmatrix}
    1       & \nicefrac{1}{2} \\
    \nicefrac{1}{2}       & 1
\end{bmatrix} \begin{bmatrix}
    x \\
    p_{3}
\end{bmatrix} - \begin{bmatrix}
    \hat{x} \\
    \hat{p_3}
\end{bmatrix}^T \begin{bmatrix}
    1       & 0 \\
    0       & 1
\end{bmatrix} \begin{bmatrix}
   2\cdot x- \hat{x} \\
   2 \cdot p_{3} - \hat{p_3}
\end{bmatrix},  \\		
&  \delta_{0}\geq 0 , \quad \delta_{1}\geq 0 , \quad \delta_{2} \geq 0. 
		\end{align*}
\end{example}
If all penalty variables are assigned to zero, we may terminate the loop in \cref{fig:ccploop}.
\begin{theorem}
	\label{thm:main}
	For a pMDP $\pmdp$, property $\varphi$, and corresponding convex DC problem \cref{constr:qcqp:final}, it holds that a satisfying assignment $\val$ of the DC problem with 
	\begin{align*}
		\Big(\tau\sum_{\forall s\in S\setminus T}\sum_{\forall \act \in \Act}\delta_{s,\act}\Big)[\val]=0		
	\end{align*}
 accepts $\varphi$ on $\pmdp$ (under demonic nondeterminism).
\end{theorem}
\begin{proofsketch}
Let $\val$ be a satisfying valuation as in the theorem.
With the side condition on the penalty variables, the constraints in \cref{constr:qcqp:final} reduce to the constraints in \cref{constr:qcqp:overapproxdc}. 
From \cref{prop:qcqp:overapprox} we conclude that  the valuation is also satisfying the constraints from \cref{constr:qcqp:dc}. Via \cref{cor:qcqp:dcreformulation}, the valuation satisfies the constraints from \cref{constr:ubreachgpdnondet}.
Using the results from \cref{sec:parametric:etr}, the valuation accepts $\varphi$ on $\pmdp$.
The technical report of \cite{DBLP:conf/atva/CubuktepeJJKT18} contains an alternative  proof.
\end{proofsketch}

\paragraph{Update}
If any of the penalty variables are assigned to a positive value, we update the penalty parameter $\tau$ by $\mu + \tau$ for a $\mu > 0$, until an upper limit for $\tau_{\mathit{max}}$ is reached to avoid numerical problems.
Then, we compute a linearization of the $g_i$ functions around the current (not feasible) solution and solve the resulting problem. 
This procedure is repeated until we find a feasible solution. 
The procedure may get stuck:
Small violations of the original over-approximating DC, i.e., small $\delta_{s,\act}$ values may lead to big differences in the actual computed $p_\init$.
Then, the CCP may be stuck in poor local optima, where the sum of constraint violations is small, but the violation for the probability threshold is too large.
We circumvent the problem as follows: if the procedure converges to an infeasible solution, it may be restarted with adapted initial values $\hat{v}$.



\paragraph{Eigenvalue-less DP}

We may use the transformation in Equation~\eqref{eq:makepsd}, but it involves expensive matrix operations, including computing the numerous eigenvalues to make the matrix PSD.
Observe that 
the matrices $\qcqpmatrix_{s,\act}$ and vectors $q_{s,\act}$ are sparse. 
Then, the eigenvalue method introduces more occurrences of the  variables in every constraint 
 and thereby increases the approximation error during convexification. 

We use an alternative convexification which is based on the observation that the quadratic monomials are bilinear---state variables and parameters are never squared.
Consider the bilinear polynomial $h \coloneq 2c\cdot yz$, where $y$ and $z$ are variables and $c \in \RRpos$.
We rewrite $h$ equivalently using \[ h \rightsquigarrow  h + c(y^2+z^2) - c(y^2+z^2).\]
Then, we rewrite $h + c(y^2+z^2)$ as $2c\cdot yz + c(y^2+z^2) = c(y+z)^2$.
We obtain \[ h = c(y+z)^2 -c(y^2+z^2).\]
The function $c(y+z)^2$ is a quadratic convex polynomial and we convexify the polynomial $-c(y^2+z^2)$  as $-c(\hat{y}^2+\hat{z}^2)+2c(\hat{y}^2+\hat{z}^2-y \hat{y} - z \hat{z}),$ where $\hat{y}$ and $\hat{z}$ are the assignments as before.
Together, this yields the following reformulation into a convexified constraint:
\[ 2c\cdot yz \rightsquigarrow c(y+z)^2 -c(\hat{y}^2+\hat{z}^2)+2c(\hat{y}^2+\hat{z}^2-y\cdot\hat{y} - z \cdot\hat{z}). \]

% in Sect.~\ref{subsec:ccpprocedure}. 
We convexify the bilinear polynomial  $h = 2c\cdot yz$ with $c \in \RRneg$ analogously
 by adding and subtracting the concave function $-c(y^2+z^2)$ to rewrite $2cyz$ as $-c(y-z)^2+c(y^2+z^2)$. 
%Then, again analogously, the concave function $c(y^2+z^2)$, can be convexified as $c(\hat{y}^2+\hat{z}^2)-2c(\hat{y}^2+\hat{z}^2-y \hat{y} - z \hat{z})$.
Consequently, we reduce the occurrences of variables for sparse matrices compared to the eigenvalue method.


\paragraph{Tuning magic constants.}
Optimally, we would initialise the CCP procedure, i.e., values $\hat{v}$ (for the parameters and the state variables) with a feasible valuation, but that would require to already solve the feasibility problem itself.
Instead, we instantiate the $\hat{x}$ components of $\hat{v}$ as the centre of the parameter space, and thereby minimise the worst-case distance to a feasible solution.
For $\hat{p_s}$, we use the threshold $\lambda$ from the specification to initialise the probability variables, and analogously for expected cost.
We initialise the penalty constant $\tau\coloneq0.05$ for reachability, and $\tau\coloneq5$ for expected cost, a conservative number in the same order of magnitude as the values $\hat{p_s}$.
As expected cost evaluations have wider ranges than probability evaluations, a larger $\tau$ is sensible.
We pick $\mu \coloneq \max_{s\in S\setminus T } \hat{p_s}$.
We update $\tau$ by adding $\mu$ after each iteration. 
Empirically, increasing $\tau$ with bigger steps is beneficial for the run time, but induces more numerical instability.
In contrast, in the literature, the update parameter $\mu$ is frequently used as a constant, i.e., it is not updated between the iterations. 
In, e.g,~\cite{lipp2016variations}, $\tau$ is multiplied by $\mu$ after each iteration. 

\subsection{Integration with model checking}

\begin{figure}
\centering
\tikzsetnextfilename{qcqpmcloop}
	\input{figures/qcqpmcloop}
	\caption{CCP and model checking in the loop}
	\label{fig:ccpwithmc}
\end{figure}

\paragraph{Model checking in the loop}
The first and foremost assumption, backed by experiments, is that model checking single instantiations of a pMDP is much faster than an iteration of the CCP.
Consequently, we slightly change the loop from \cref{fig:ccploop} to the loop in \cref{fig:ccpwithmc}, making two changes.
The first change is that we no longer check the penalty of a solution.
Instead, we use the values $\val(x)$ for each $x \in \pars$, which give rise to a parameter valuation.
Model checking at these instantiations has two benefits:
First, it allows for \emph{early termination}. 
We check whether $\instantiated{\pmdp}{\val}$ accepts $\varphi$: If yes, we have found a solution even though the penalty variables have not converged to zero.
Second, the model checking procedures are numerically more stable and allow for exact arithmetic. Thereby, the solutions are more reliable than the solutions obtained from the convex solver.

The second change is in the update procedure.
Using the model checking results often overcomes convergence to infeasible solutions.
These problems may be described as follows:
Instead of instantiating the initial probability value for the next iteration as $\hat{p_s} \coloneq \val(p_s)$, we may use the model-checking result $\mathsf{res}$ of the MDP $\instantiated{\pmdp}{\val}$ and set $\hat{p_s} \coloneq \mathsf{res}(s)$. 
Model checking ensures that the probability variables are consistent with the parameter variables, i.e., that the constraints describing the transition relation in the original encoding are all satisfied.

 
\paragraph{Algorithmic improvements} 
We list three technical  improvements that significantly improved the performance of the approach.
\begin{inparaenum}[(1)]
\item 	
We precompute zero-states and one-states and simplify the constraints accordingly.
\item
For simple(x) pMDPs, the well-formed constraints are written compactly.
\item 
Parts of the encoding are untouched over multiple CCP iterations.
% specifically the constraints with affine functions.
Instead of rebuilding the encoding, we only update constraints which contain iteration-dependent values. 
The update is based on a preprocessed representation of the model.
The improvement is two-fold: We spend less time constructing the encoding and the solver reuses previous results, making solving up to three times faster.
\end{inparaenum} 



\section{Empirical Evaluation}

\subsection{Set-up}
\paragraph{Implementation}
We implement the CCP with the above mentionend efficiency improvements in the parameter synthesis framework \prophesy.
We use the probabilistic model checker \storm~\cite{DBLP:conf/cav/DehnertJK017} to extract an explicit representation of  a pMDP.
We keep the pMDP in memory and update the parameter instantiations using an efficient data structure to enable efficient repetitive model checking.
To solve convex QCQPs, we use \Gurobi{} 7.5~\cite{gurobi}, configured for numerical stability.


\paragraph{Environment}
We evaluate on a HP BL685C G7 with 48 2 GHz cores, a 32 GB memory limit, and 1800 seconds time limit; the implementation uses a single thread.

\paragraph{Settings}
We consider feasibility, i.e., the task is to find feasible parameter valuation for pMCs and pMDPs with non-trivial upper/lower thresholds on probabilities/rewards in the property.
We ask for a  $\varepsilon$-preserving valuation of the parameters, with $\varepsilon\coloneq10^{-5}$.
We run all the approaches with the exact same configuration of \storm. 
For pMCs, we enable weak bisimulation, which is beneficial for all presented examples. 
We do not use bisimulation for pMDPs.

\paragraph{Base line}
We compare runtimes with a particle-swarm optimisation (PSO, \cref{sec:sampling}) and the SMT-based approaches (direct or via solution function, \cref{sec:useetr}).
As PSO is a randomised procedure, we run it with random seeds 0--19. 
The PSO implementation requires the well-defined parameter regions to constitute a hyper-rectangle, as proper sampling from polygons is a non-trivial task.

We additionally compare against a prototype of the geometric programming (GP) approach~\cite{DBLP:conf/tacas/Cubuktepe0JKPPT17} based on CvxPy~\cite{DBLP:journals/jmlr/DiamondB16} and the solver SCS~\cite{DBLP:journals/jota/ODonoghueCPB16}, and the QCQP package~\cite{parkqcqp2017}, which implements several heuristics, including a naive CCP approach, for nonconvex QCQPs. 
Due to numerical instabilities, we failed to automatically and successfully apply these two approaches to a wide range of benchmarks.


\paragraph{Benchmarks}
We include the standard pMC benchmarks from the \PARAM website, which contain two parameters.
We consider a large set of POMDP strategy synthesis problems from \cref{sec:pomdps}:
\textsl{GridX} are gridworld problems with trap states (A), finite horizons  (B), or movement costs (C). 
\textsl{Maze} is a navigation problem.
\textsl{Netw} and \textsl{Repud} originate from distributed protocols, and were included in \cite{DBLP:journals/rts/Norman0Z17}.
We obtain the pMDP benchmarks either from the \PARAM{} website, or as parametric variants to existing \prism{} case studies, and describe randomised distributed protocols.


\subsection{Evaluation}

\subsubsection{Experiments}

\paragraph{Results}%\mc{moved pmdp bisimulation stuff to the setup paragraph}\nj{good}

\begin{table}[t]
\centering
\footnotesize{
\caption{pMC benchmark results}
\label{tab:results_pmc}
\begin{tabular}{lll|rrr|rrr|r|rrr}
\multicolumn{3}{c|}{Problem} & \multicolumn{3}{c|}{Info} & \multicolumn{3}{c|}{PSO} & SMT & \multicolumn{3}{c}{CCP} \\
Set    & Inst    & Spec   & States   & Trans.  & Par.      & tmin   & tmax   & \textbf{tavg}  & \textbf{t}   & \textbf{t}    & solv    & iter    \\\hline
% Crowds
\textsl{BRP}  & 16,2         & $\probop{\leq 0.1}{}$       & 98    & 194  & \highlight{2}     &  0     & 0       &  \textbf{0}     & 40    & 0     &  30\%  &   3 \\
\textsl{BRP}  & 512,5         & $\probop{\leq 0.1}{}$      & 6146    & 12290  & \highlight{2}     &  24     & 36       &  \textbf{28}     & \TO    & 33     &  24\%  &   3 \\
% Crowds
\textsl{Crowds}  & 10,5         & $\probop{\leq 0.1}{}$      & 42    & 82  & \highlight{2}     &  4     & 5       &  5     & 8    & \textbf{4}     &  2\%  &   4 \\
% Nand
\textsl{Nand}  & 5,10         & $\probop{\leq 0.05}{}$      & 10492    & 20982  & \highlight{2}     &  21     & 51       &  28     & \TO    & \textbf{22}     &  21\%  &   2 \\
% Zeroconf
\textsl{Zeroconf}  & 10000         & $\rewop{\leq 10010}{}$      & 10003    & 20004  & \highlight{2}     &  2      & 4       &  \textbf{3}     & \TO    & 57     &  81\%  & 3  \\\hline
%4x4grid_avoid_sl_simple_m4.drn
\textsl{GridA}  & 4         & $\probop{\geq 0.84}{}$      & 1026    & 2098  & \highlight{72}     &   11     &   11     &  \textbf{11}     &  \TO    & 22     &  81\%  & 11  \\
%4x4grid_bounded_8_sl_simple_m5.drn
\textsl{GridB}  & 8,5         & $\probop{\geq 0.84}{}$      & 8653    & 17369  & \highlight{700}     &    409    &   440     & 427      & \TO    & \textbf{213}     &  84\%  & 8  \\
%4x4grid_bounded_10_sl_simple_m6.drn
\textsl{GridB}  & 10,6         & $\probop{\geq 0.84}{}$      & 16941    & 33958  & \highlight{1290}     &  533      &   567     &  553     &  \TO   & \textbf{426}     &  84\%  & 7  \\
%grid4x4_simple_extended_m6.drn
\textsl{GridC}  & 6         & $\rewop{\leq 4.8}{}$      & 1665    & 305  & \highlight{168}     &  261      &  274      &  267     &  \TO   & \textbf{169}     &  90\%  & 23  \\
%maze_simple_extended_m5.drn  
\textsl{Maze}  & 5         & $\rewop{\leq 14}{}$      & 1303    & 2658  & \highlight{590}     &  213  & 230 & 219         &  \TO   &   \textbf{67}   &  89\%  & 8  \\
%maze_simple_extended_m5.drn  
\textsl{Maze}  & 5         & $\rewop{\leq 6}{}$      & 1303    & 2658  & \highlight{590}     &     -- &  -- & {\TO}          &  \TO   & \textbf{422}     &  85\%  & 97  \\

%maze_simple_extended_m7.drn  
\textsl{Maze}  & 7         & $\rewop{\leq 6}{}$      & 2580    & 5233  & \highlight{1176}     &    -- &  -- & {\TO}      & \TO    & \textbf{740}     &  90\%  & 60  \\
% network_T5_simple_extended_m2
\textsl{Netw}  & 5,2         & $\rewop{\leq11.5}{}$      & 21746    & 63158  & \highlight{2420}     &  312      & 523       &   359    &  \TO   & \textbf{207}     & 39\%   & 3  \\

% network_T5_simple_extended_m2
\textsl{Netw}  & 5,2         & $\rewop{\leq10.5}{}$      & 21746    & 63158  & \highlight{2420}     &        -- &  -- & {\TO}        &  \TO   & \textbf{210}     & 38\%   & 4  \\
% network_T4_simple_extended_m3
\textsl{Netw}  & 4,3         & $\rewop{\leq11.5}{}$      & 38055    & 97335  & \highlight{4545}     &        -- &  -- & {\TO}        &  \TO   & \MO     & -   & -  \\

% repudiation_simple_extended_m5.drn
\textsl{Repud}  & 8,5         &   $\probop{\geq 0.1}{}$     & 1487    & 3002  & \highlight{360}     &   16     & 22       &   18    & \TO    & \textbf{4}     & 36\%   & 2  \\
% repudiation_simple_extended_m5.drn
\textsl{Repud}  & 8,5         & $\probop{\leq 0.05}{}$       & 1487    & 3002  & \highlight{360}     &    273    &   324     &   293    &  \TO   & \textbf{14}     &  72\%  &  4 \\
%repudiation_16_simple_extended_m2
\textsl{Repud}  & 16,2         &  $\probop{\leq 0.01}{}$     & 790    & 1606  & \highlight{96}     &       -- &  -- & {\TO}       & \TO    &  \textbf{15}    & 78\%   & 9  \\
\textsl{Repud}  & 16,2         &  $\probop{\geq 0.062}{}$     & 790    & 1606  & \highlight{96}     &       -- &  -- & {\TO}       & \TO    &  \TO    & -   & -  \\\hline


\end{tabular}
}
\end{table}

\cref{tab:results_pmc} contains an overview of the results for pMCs.
The first two columns refer to the benchmark instance, the next column to the specification evaluated. 
We give the states (States), transitions (Trans.) and parameters (Par.) \emph{in the bisimulation quotient}, which is then used for further evaluation.
We then give the \emph{minimum} (tmin), the \emph{maximum} (tmax) and \emph{average} (\textbf{tavg}) runtime (in seconds) for PSO with different seeds, the best runtime obtained using SMT (\textbf{t}), and the runtime for CCP (\textbf{t}). 
For CCP, we additionally give the fraction (in percent) of time spent in \Gurobi{}  (solv), and the number of CCP iterations (iter).
\cref{tab:results_pmdp} reports on the results for pMDPs and additionally contains the number of actions (Act) for pMDPs.
The boldfaced measures \textbf{tavg} and \textbf{t} for both SMT and CCP are the important measures to compare. 
Boldface values are the ones with the best performance for a specific benchmark.

\begin{table}[t]
\centering
\caption{pMDP benchmark results}
\label{tab:results_pmdp}
\footnotesize{
\begin{tabular}{lll|rrrr|rrr|r|rrr}
\multicolumn{3}{c|}{Problem} & \multicolumn{4}{c|}{Info}   & \multicolumn{3}{c|}{PSO} & SMT & \multicolumn{3}{c}{CCP} \\
Set    & Inst    & Spec   & States & Act & Trans. & Par. & tmin   & tmax   & \textbf{tavg}  & \textbf{t}   & \textbf{t}    & solv    & iter    \\\hline


\textsl{BRP} & 4,128 & $\probop{\leq 0.1}{}$&17131 & 17396 & 23094 & \highlight{2}  & 45 & 47 & 46 & \TO & \textbf{39}
 & 33\%  & 4 \\  
\textsl{Coin} & 32 &$\rewop{\leq 500}{}$& 4112 & 6160 & 7692 & \highlight{2} & 117 & 119 & \textbf{118} & \TO & \TO & - & - \\ 
\textsl{CoinX} & 32 & $\rewop{\leq 210}{}$& 16448 & 24640 & 30768 & \highlight{2} & 1196 & 1222 & 1208 & \TO & \textbf{32} & 78\% & 3 \\ 
%
\textsl{Zeroconf}       & 1        & $\probop{\geq 0.99}{}$& 31402      &  55678      &  70643   &    \highlight{3}   & 18    &  19      & \textbf{19}        &  \TO      &     79     &    82\%     &   2 \\
%
\textsl{CSMA} & 2,4 & $\rewop{\leq 69.3}{}$& 7958 & 7988 & 10594 & \highlight{26} & n.s. & n.s. & n.s. & \TO & \textbf{79}  & 86\% & 10  \\
\textsl{Virus} & - & $\rewop{\leq 10}{}$& 809 & 3371 & 6741 & \highlight{18} &  113 & 113 & 113 & \TO & \textbf{13} & 76\% & 4 \\
\textsl{Wlan} & 0 & $\rewop{\leq 580}{}$& 2954 & 3972  & 5202 & \highlight{15} & n.s. & n.s. & n.s. & \TO & \textbf{7} & 72\% & 2 \\\hline
 
    
\end{tabular}
}
\end{table}

\paragraph{Interpretation}
There is a constant overhead for model building, which is in particular large if the bisimulation quotient computation is expensive, see the small fraction of time spent solving DPs for \textsl{Crowds}.
For the more challenging instances, this overhead is negligible. Roughly 80--90\% of the time is spent within \Gurobi{}  for these instances, the remainder is used to feed the DPs into \Gurobi.
A specification threshold closer to the (global) optimum typically induces a higher number of iterations (see \textsl{Maze} or \textsl{Netw} with different thresholds).
For the pMDP \textsl{Coin}, optimal parameter values are on the boundary of the parameter space and are quickly reached by PSO. The small parameter values together with the rather large expected costs are numerically challenging for CCP. 
 For \textsl{CoinX}, the parameter values are in the interior of the parameter space and harder to hit via sampling. 
 For CCP, the difference between small and large coefficients is smaller than in \textsl{Coin}, which yields better convergence behaviour.
 The benchmarks \textsl{CSMA} and \textsl{WLAN} are currently not supported by PSO due to the non-rectangular well-defined parameter space.
 CCP does not solve all instances: 
In \textsl{Netw} (4,3), CCP exceeds the memory limit.
In \textsl{Repud}, finding values close the global optimum requires too much time. 
While the thresholds used here are close to the global optima, actually finding the global optimum itself is always challenging.


\paragraph{Effect of integrating model checking for CCP} 
A naive CCP method without model checking mostly yields an inferior performance for our synthesis problem.

The benchmark-set \textsl{Maze} profits most: 
Discarding the model checking results in our CCP implementation always yields time-outs, even for the rather simple \textsl{Maze} with threshold 14, which is solved with usage of model checking results within 70 seconds.
Here, using model checking results thus yields a speed-up by a factor at least 25.
More typical examples are \textsl{Netw}, where discarding the model checking results yields a factor five performance penalty.
The \textsl{Repud} examples do not significantly profit from using intermediate model checking results.

\paragraph{Evaluation of the QCQP package, GP and SMT}%\mc{this paragraph is in past tense, change it to present?}
We evaluate the GP on pMCs with two parameters: 
For the smaller \textsl{BRP} instance, the procedure takes 90 seconds, for \textsl{Crowds} 14 seconds. Other instances yield timeouts. 
We also evaluate the QCQP package on some pMCs. 
For the smaller \textsl{BRP} instance, the package takes 113 seconds, and 13 seconds for the \textsl{Crowds}. 
For a \textsl{Repud} instance with 44 states, %110 transitions,
 and 26 parameters, the package takes 54 seconds and returns a rejecting valuation. 
 Our CCP-loop with integrated model checking takes less than a second.

The results in \cref{tab:results_pmc} and~\ref{tab:results_pmdp} make obvious that \emph{SMT is not competitive}, irrespectively whether the formula is preprocessed via state elimination.
Moreover, state elimination (for pMCs) within the given time limit \emph{is only possible for the (considered) models with 2 parameters}, using either \prism, \PARAM, or \storm. 

\subsubsection{Discussion}
Based on the empirical evaluation, we make the following claims.
\paragraph{A tuned variant of CCP improves the state-of-the-art.}
Just applying out-of-the-box heuristics for QCQPs---like realised in the QCQP package or using our CCP implementation without integrated model checking---does not yield a scalable method.
To solve the nonconvex QCQP, we require a CCP with a clever encoding and several algorithmic improvements.
%In fact, integrating model checking techniques is the key.
State space reductions shrink the encoding and model checking after each CCP iteration to terminate earlier typically saves 20\% of iterations. 
Especially when convergence is slow, model checking saves significantly more iterations.
Moreover, feeding model checking results into the CCP improves the runtime by up to an additional order of magnitude, at negligible costs. 
%Together, a CCP based approach improves the state-of-the-art. 
These combined improvements to the CCP method outnumbers any solver-based approach by orders of magnitude and is often superior to sampling based approaches, especially in the presence of many parameters.
Benchmarks with many parameters pose two challenges for sampling based approaches: 
Sampling is necessarily sparse due to the high dimension and
%the effect of parameter values are interdependent.
 optimal parameter valuations for one parameter often depend significantly on other parameter values.
 % of other parameters. \sj{Hard to grasp sentence}  

\paragraph{CCP performance can be boosted with particular benchmarks in mind.}
For most benchmarks, choosing larger values for $\tau$ and $\mu$ improves the performance. 
Furthermore, for particular benchmarks, we can find a better initial valuation $\hat{v}$. 
These adaptions, however, are not suitable for a general framework. 
We have chosen magic constants that reflect a more balanced performance over several types of benchmarks.
On the downside, the dependency on the constants means that minor changes in the encoding may have a significant, but hard to predict, effect.
For SMT-solvers, additional and superfluous constraints often help steering the solver, but in the context of CCP, it deteriorates the performance.

\paragraph{Some benchmarks constitute numerically challenging problems.}
For specification thresholds close to global optima and for some expected cost specifications in general, feasible parameter values may be tiny. 
Such extremal parameter values induce CCPs with large differences between the smallest and largest coefficient in the encoding and are numerically challenging.
The pMDP benchmarks seem more susceptible to such numerical issues.

\begin{introconclbox}
Affine pMDPs cover most pMDP benchmarks, and the ETR encoding for them is bilinear. This observation allows using dedicated (numerical) solvers to find feasible valuations. Crucially, it allows us to adapt the CCP technique. Intuitively, we accelerate sampling by solving a convex approximation of the original constraint system around each sample.
Using this adapted CCP approach not only outperforms methods that rely purely on the ETR encoding, but also the sampling-based PSO method.
\end{introconclbox}




==> convex_optimization.tex <==
\section{Parameter/strategy synthesis for probabilistic systems using nonlinear optimization}
\nj{restrict rational functions to the ones we can handle.}
We are given a parametric Markov chain (pMC) $\dtmcInit$ with $P\colon S\times S\rightarrow\functions[\Var]$ for $\functions[\Var]$ being the set of \emph{rational functions} over a finite set of parameters $\Var$. 
Adding nondeterminism, assume a parametric Markov decision process pMDP $\MdpInit$ with $\probmdp \colon S \times \Act \times S \rightarrow \functions[\Var]$. For both $\dtmc$ and $\mdp$ we are given a set of target states $T\subseteq S$ and a unique initial state $\sinit\in S$.

There are several measures of interest: 
\begin{enumerate}
	\item For a pMC $\dtmc$, find a \emph{parameter valuation} for $\Var$ that induces the minimal or maximal probability or expected cost to reach $T$ 
	\item For a pMDP $\mdp$, find a parameter valuation and a \emph{scheduler} inducing again minimal or maximal probability or expected cost to reach $T$.
	\item For a given valuation $u$ of parameters and either a pMC $\dtmc$ or a pMDP $\mdp$, find a new valuation $u'$ \emph{minimally deviating} from $u$ such that a certain property for $\dtmc$ or $\mdp$ is satisfied which was violated before. (This is referred to as model repair~\cite{bartocci2011model}).
	\item For an MDP and multiple objectives, find a \emph{randomized scheduler} that induces satisfaction of all objectives. This problem was studied in~\cite{DBLP:journals/lmcs/EtessamiKVY08,DBLP:conf/atva/ForejtKP12}. To distinguish ourselves from these results, we investigate scenarios where it makes sense to impose restrictions on schedulers, \ie dependencies of randomized decisions at different states.
	\nj{I need to check how optimality is defined for multiple objectives.}
\end{enumerate}


%\emph{Strategy variables} $\sigma^{s,\act}\in[0,1]$ for each state $s\in S$ and action $\act\in\Act$ define a strategy $\sigma$ by $\sigma(s,\act)=\sigma^{s,\act}$ if additional side constraints ensure well-definedness. 
%Analogously, \emph{perturbation variables} $\delta^{s,\act}\in[-1,1]$ define a perturbation via $\delta(s,\act)=\delta^{s,\act}$ for all $s\in S$ and $\act\in\Act$.	
%

		
\subsection{Nonlinear optimization/feasibility problems}
In the following we list the problems for MCs and MDPs, restricting ourselves to reachability probabilities.
\subsubsection{A. Markov chains.}
Let $\dtmc$ be a pMC. We assume that all transition probabilities are either constant probabilities or are of the form $p$ for $p\in\Var$. If a transition probability is, \eg, of the form $1-p$, we substitute it by a fresh parameter $\overline p$ which we add to $\Var$. In that case we have to ensure that assignments of parameters induce that at each state the probabilities sum up to one.

In addition to the parameters from $\Var$, we introduce the following \emph{variables}:
		\begin{itemize}
			\item $p_s\in[0,1]$ for each $s\in S$ will be assigned the probability of reaching $T\subseteq S$.
		\end{itemize}
	 	The NLP for maximizing the probability of reaching $T$ reads as follows:
		\begin{align}
			\text{maximize } &\quad p_{\sinit}\label{eq:min}\\
			\text{such that}\\
%							 &\quad p_{\sinit}\leq \lambda\label{eq:strategyah:lambda}\\
			\forall s\in T.	 &\quad p_s=1\label{eq:targetprob}\\
			\forall s\in S\setminus T.	&\quad p_s = \sum_{s'\in S}	P(s,s')\cdot p_{s'}\label{eq:probcomputation}\\
			\forall s\in S.	 &\quad \sum_{s'\in S}P(s,s')=1\label{eq:well-defined_probs}
		\end{align}
		Constraint~\ref{eq:well-defined_probs} enforces that parameters are assigned values in a way such that well-defined probability distributions result. 
		
\subsubsection{B. Markov decision processes---deterministic schedulers.}
Let $\mdp$ be an MDP. We again use the following \emph{variables}:
		\begin{itemize}
			\item $p_s\in[0,1]$ for each $s\in S$ will be assigned the probability of reaching $T\subseteq S$.
		\end{itemize}
	 	The NLP reads as follows:
		\begin{align}
			\text{minimize } &\quad p_{\sinit}\label{eq:min_mdp}\\
			\text{such that}\\
%							 &\quad p_{\sinit}\leq \lambda\label{eq:strategyah:lambda}\\
			\forall s\in T.	 &\quad p_s=1\label{eq:targetprob_mdp}\\
			\forall s\in S\setminus T.\,\forall \act\in\Act.	&\quad p_s \geq \sum_{s'\in S}	\probmdp(s,\act,s')\cdot p_{s'}\label{eq:probcomputation_mdp}\\
			\forall s\in S.\, \forall\act\in\Act.	 &\quad \sum_{s'\in S}\probmdp(s,\act,s')=1\label{eq:well-defined_probs_mdp}
		\end{align}
Note that this optimization problem computes the \emph{maximal probability} of reaching T under a deterministic scheduler. The reachability probabilities for each choice of action are put as a lower bound to the probability variables $p_s$ for each $s\in S$. In order for the assignment to satisfy the highest lower bound with equality, $p_{\sinit}$ is minimized. If the minimal probability is to be found, the probabilities need to be put as upper bound while $p_{\sinit}$ is maximized.

\subsubsection{C. Markov decision processes---randomized schedulers.}
For some properties, in particular when having multiple objectives, randomized schedulers are strictly more powerful than deterministic ones. For the NLP, we introduce the following specific \emph{variables}:
		\begin{itemize}
			\item $\sched^{s,\alpha}\in[0,1]$ for each $s\in S$ and $\act\in\Act$ define the randomized scheduler $\sched$. Note that these scheduler variables may be assigned zero.
			\item $p_s\in[0,1]$ for each $s\in S$ will be assigned the probability of reaching $T\subseteq S$ from state $s$ under strategy $\sched$.
		\end{itemize}
	 	The NLP reads as follows:
		\begin{align}
			\text{minimize } &\quad p_{\sinit}\label{eq:min_rand}\\
			\text{such that}\\
%							 &\quad p_{\sinit}\leq \lambda\label{eq:strategyah:lambda}\\
			\forall s\in T.	 &\quad p_s=1\label{eq:targetprob_rand}\\
			\forall s\in S.	&\quad \sum_{\act\in\Act}\sched^{s,\act}=1\label{eq:welldefined_sched_rand}\\
			\forall s\in S\setminus T.	&\quad p_s=\sum_{\act\in\Act}\sigma^{s,\act}\cdot\sum_{s'\in S}	\probmdp(s,\act,s')\cdot p_{s'}\label{eq:probcomputation_rand}\\
			\forall s\in S.\, \forall\act\in\Act.	 &\quad \sum_{s'\in S}P(s,\act,s')=1\label{eq:well-defined_probs_rand}
		\end{align}
	\paragraph{Further specifications.}
We now explain how the NLP can be extended for further specifications. Assume  another reachability probability for target states $T'$ with $T'\neq T$ is of interest. We add another set of probability variables $p'_s$ for each state $s\in S$; Equation~\eqref{eq:targetprob_rand} is defined for all states $s\in T\cup T'$ and~\eqref{eq:probcomputation_rand} is copied for all $p'_s$, thereby computing the probability of reaching $T'$ under the same scheduler as for reaching $T$. It mostly makes sense, to optimize the probability of only one objective; therefore we assume for any further reachability objective to have a reachability specification to be satisfied, \eg, $\reachProp{\lambda}{T'}$.

	To handle an \emph{expected cost property} $\expRewProp{\kappa}{G}$ for $G\subseteq S$, we use variables $r_s$ being assigned the expected cost for reaching $G$ for all $s\in S$. We add the following equations:
%	
	\begin{align}
							 &\quad r_{\sinit}\leq \kappa\label{eq:strategyahexp:kappa}\\
			\forall s\in G.	 &\quad r_s=0\label{eq:strategyahexp:targetrew}\\
			\forall s\in S.	&\quad r_s= \sum_{\act\in\Act} \Bigl(\sigma_{ha}^{s,\act} \cdot \rew(s,\act) +    \sum_{s'\in S}	\probmdp (s,\act)(s') \cdot r_{s'}\Bigr)\label{eq:strategyahexp:rewcomputation}	
		\end{align}
		First, the expected cost of reaching $G$ is smaller than or equal to $\kappa$ at $\sinit$~\eqref{eq:strategyahexp:kappa}. Goal state are assigned cost zero~\eqref{eq:strategyahexp:targetrew}, otherwise infinite cost is collected at absorbing states. Finally, the expected cost for all other states is computed by~\eqref{eq:strategyahexp:rewcomputation} where according to the blended strategy $\sched_{ha}$ the cost of each action is added to the expected cost of the successors. 
	An important insight is that if all specifications are expected reward properties, the program is \emph{no longer nonlinear} but a linear program (LP), as there is no multiplication of variables.
%

\medskip

\subsubsection{Feasibility problems.} In case one is not interested in the exact minimal (or maximal) probability, we can also impose upper or lower bounds $\lambda\in\R$ on the reachability probability:
		\begin{align}
		p_{\sinit}\leq\lambda\\
		p_{\sinit}\geq\lambda
		\end{align}
		If we want to determine feasibility within certain \emph{parameter regions}, we can also add constraints restricting the valuations of parameters, \eg, 
	\begin{align}
		\forall x\in \Var.	 &\quad a_x\leq x\leq b_x\label{eq:region}
	\end{align}
	for $a_x,b_x\in[0,1]$ for all $x\in\Var$.
		Together with such restrictions on parameter valuations, this can help to find out if inside such a region there exists one valuation satisfying/violating the given reachability specification. This is a nonlinear feasibility problem and can be solved by SMT solvers like \tool{Z3}~\cite{demoura_nlsat}.
		
		

\section{Utilizing convex optimization}

\paragraph{Geometric programming}
In~\cite{boyd_convex_optimization}, it is described how a nonlinear program of a special form, called \emph{geometric program}, can be transformed into a convex optimization problem. We want to make use of this transformation.
Let $x=\{x_1,\ldots,x_n\}$ be a set of variables with $x_i\in\R_{>0}$ for $1\leq i\leq n$. Let $h(x)$ denote a \emph{monomial} over $x$ and $f(x)$ denote a \emph{posynomial} over $x$, as in~\cite{boyd_convex_optimization}. \nj{Add details.}

A \emph{geometric program} is of the form
\begin{align}
	\text{minimize} 		&\quad f_0(x)\\
	\text{such that} 		&\\
	\forall i.\, 1\leq i\leq m 	&\quad f_i(x)\leq 1\\
	\forall i.\, 1\leq i\leq p 	&\quad h_i(x)= 1
\end{align}
Summarized, only real-valued, positive variables are allowed. All posynomials are upper bounded by one, all monomials are equal to one, and the objective function is a posynomial.



\paragraph{Thoughts on the transformation.}
First, recall that in order for a nonlinear program to be geometric, all variables need to be positive.
For \emph{probability variables} $p_s$, we have to ensure that the computed strategy ensures a positive reachability probability for target states \emph{for all states}. We consider the following cases for pMCs:
\begin{itemize}
	\item \textit{Prob0}-states: There exists on path from these states to the target states $T$, \ie for $s\in\textit{Prob0}$ the probability to reach $T$ is $0$ and $p_s=0$ needs to hold. These states are removed from the pMC. Note that this might leave substochastic distributions at the predecessor states.
	\item \textit{Prob1}-states: The probability to reach $T$ is $1$. As a preprocessing, these states can be added to $T$ and made absorbing.
\end{itemize}
For pMDPs, we have the following cases:
\begin{itemize}
	\item \textit{Prob0A}-states: For all schedulers, the probability of reaching $T$ is $0$. As before, these states can be removed.
	\item \textit{Prob0E}-states: For these states, there exists a scheduler that induces probability $0$ of reaching $T$. In~\cite{wimmer-et-al-tcs-2014}, we called these states \emph{problematic} and offered an SMT/MILP encoding to avoid that the problematic schedulers are assigned. Note that in case of maximizing the reachability probability of target states, this is not a problem as problematic schedulers will never be chosen. For feasibility problems, however, we might need to handle this problem. 
	\nj{Are constraints enforcing reachability of target states possible in geometric program?}
\end{itemize}
All these sets of states can be computed by simple graph analysis of the pMC/pMDP.


%Algorithmically, this can be achieved by a preprocessing in the following way: Compute the set of \emph{problematic states} for $\mdp$, \ie, the set of states where a strategy exists that induces probability zero of reaching target states. For these states, inside the NLP encoding, reachability has to be ensured, see~\cite{wimmer-et-al-tcs-2014}.

In addition to the probability variables, also for \emph{strategy variables} $\sched^{s,\act}$ it is now no longer allowed to have probability zero for an action at state $s$, \ie, $\sched^{s,\act}=0$. One idea could be to ensure a \emph{minimal probability} $p_\epsilon$ to be assigned for all actions at each state. Getting exactly this minimal probability as a result might hint to the fact that actually $0$ induces the optimal solution.

\subsubsection{Equality constraints}
The foremost problem in our setting is, that we have a lot of equality constraints in the original NLP encodings. Recall the problem of computing maximal probabilities for an MDP with deterministic strategies. Basically, we need to relax Equation~\eqref{eq:well-defined_probs_mdp}, resulting in the following geometric program:
\begin{align}
			\text{minimize } &\quad p_{\sinit}\label{geo:eq:min_mdp}\\
			\text{such that}\\
%							 &\quad p_{\sinit}\leq \lambda\label{eq:strategyah:lambda}\\
			\forall s\in T.	 &\quad p_s=1\label{geo:eq:targetprob_mdp}\\
			\forall s\in S\setminus T.\,\forall \act\in\Act.	&\quad \sum_{s'\in S}\frac{\probmdp(s,\act,s')\cdot p_{s'}}{p_s}\leq 1 \left(\Leftrightarrow p_s \geq \sum_{s'\in S} P(s,s')\cdot p_{s'}\right)\label{geo:eq:probcomputation_mdp}\\
			\forall s\in S.\, \forall\act\in\Act.	 &\quad \sum_{s'\in S}\probmdp(s,\act,s')\leq 1\label{geo:eq:well-defined_probs_mdp}
		\end{align}
In fact, the optimal solution to this problem is also an optimal solution to the original problem iff 
Equation~\ref{geo:eq:well-defined_probs_mdp} is satisfied with equality.
\nj{relate to boyd tutorial}
Note that constraints given by \eqref{geo:eq:well-defined_probs_mdp} are only generated if $\probmdp{s,\act,s'}$ is not constant. Assume now that we have $\probmdp(s,\act,s'_1)=p$ and $\probmdp(s,\act,s'_2)=1-p$. We substitute each occurrence of $1-p$ by the fresh parameter $\bar p$ and add the constraint $p + \bar p \leq 1$ which we need to be satisfied with equality. We pick $p$ which needs to have the following properties: 
\begin{enumerate}
	\item $p$ does not appear in any of the monomial constraints given by \eqref{geo:eq:targetprob_mdp}
	\item Both the objective function \eqref{geo:eq:min_mdp} and the (other) inequality constraints given by \eqref{geo:eq:probcomputation_mdp} need to be \emph{monotonically decreasing} in $p$. 
	\item The constraint generated from \eqref{geo:eq:well-defined_probs_mdp} for which $p$ was chosen needs to be \emph{monotone strictly increasing} in $p$. 
\end{enumerate}
The first and the third property are satisfied. Regarding the second property, the objective function is trivially monotonically decreasing in $p$ as the derivative of $p_{\sinit}$ with respect to $p$ is zero. The problem is \eqref{geo:eq:probcomputation_mdp}, as there will be a constraint where $p$ occurs in the numerator, rendering it monotonically increasing in $p$. Our solution is as follows: Introduce a fresh variable $p'$ which substitutes $p$ in each constraint generated by \eqref{geo:eq:probcomputation_mdp}, making the constraints (trivially) monotonically decreasing in $p$.
	Now we need to set $p$ and $p'$ into relation. Consider two programs generated either adding the constraint $p\leq p'$ or $p'\leq p$. Depending on wether $p_s$ is monoton in $p$, we can use these constraints to judge if the computed optimal probability is an upper or a lower bound on the original optimal solution. 

\subsection{Markov chains---geometric program.}
Let $\dtmc$ be a pMC. 
 We introduce the following \emph{variables}:
		\begin{itemize}
			\item $p_s\in[0,1]$ for each $s\in S$ will be assigned the probability of reaching $T\subseteq S$.
		\end{itemize}
	 	The direct adaption of the NLP in Equations~\ref{eq:min}--\ref{eq:well-defined_probs} as a geometric program reads as follows:
		\begin{align}
			\text{ minimize } &\quad \nicefrac{1}{p_{\sinit}}\\
			\text{such that}\\
%							 &\quad p_{\sinit}\leq \lambda\label{eq:strategyah:lambda}\\
			\forall s\in T.	 &\quad p_s=1\label{eq:targetprob_geo}\\
			\forall s\in S\setminus T.	&\quad  \sum_{s'\in S}	\frac{P(s,s')\cdot p_{s'}} {p_s} \leq 1\quad \left(\Leftrightarrow p_s \geq \sum_{s'\in S} P(s,s')\cdot p_{s'}\right) \label{eq:probcomputation_geo}\\
			\forall s\in S.	 &\quad \sum_{s'\in S}P(s,s')\leq 1\label{eq:well-defined_probs_geo}
		\end{align}
%
First, observe two relaxations we had to allow. First, Equation~\ref{eq:probcomputation_geo} states that $p_s \geq \sum_{s'\in S} P(s,s')\cdot p_{s'}$ for all $s\in S$, \ie, the assignment of $p_s$ is \emph{lower-bounded} by the actual probability of reaching the target states. Minimizing $p_{\sinit}$ in the objective shall push the assignment to this lower bound in order to satisfy the inequation with equality. 

Secondly, in Equation~\ref{eq:well-defined_probs_geo}, the sum of all probabilities at each state is now only upper bounded by one instead of being exactly one. This is problematic, because it might be beneficial for the objective to assign parameter values that induce sub-stochastic distributions. The first approach to remedy this is to adapt the objective function towards also maximizing the sum of all occurring parameters:
\begin{align}
			\text{ minimize } &\quad \frac{1}{p_{\sinit}} + \sum_{p\in\Var}\frac{1}{p}\label{eq:min_geo_relax1}
\end{align}

Consider the following example pMC with parameters $p$ and $\overline p = 1-p$:
\begin{figure*}
	\centering\input{pics/nonmonotonic_dtmc}	
\end{figure*}
%

We know that the probability of reaching $s_3$ from $s_0$ is given by the polynomial $f_{03}(p)=p^2-p^3$. The maximal value is at $p=\nicefrac{2}{3}$ inducing a probability of $0.1481$. State $s_4$ has probability $0$ to reach $s_3$ (\textit{Prob0}-state). It is therefore excluded, indicated by the gray outlines.

The geometric program determining this maximal reachability probability has variables $p,\overline p, p_0,p_1,p_2,p_3$ and reads as follows:
\begin{align}
			\text{ minimize } &\quad \nicefrac{1}{p_{0}} + \nicefrac{1}{p} + \nicefrac{1}{\overline p}\\
			\text{such that}\\
			&\quad p_{s_3}=1\\
			&\quad  \nicefrac{p\cdot p_{s_1}} {p_0} \leq 1\\
			&\quad  \nicefrac{\overline p\cdot p_{s_2}} {p_1} \leq 1\\
			&\quad  \nicefrac{p\cdot p_{s_3}} {p_2} \leq 1\\
			&\quad p+\overline p\leq 1\label{eq:well-defined_probs_geo}
		\end{align}

%\nj{now comes a summarizing discussion on the outcomes of this example.}

Encoding this in \tool{CVXOPT} yields an assignment $\nu$ of variables that induces sub-stochastic distributions, \ie values $\nu(p)$ and $\nu(\overline p)$ such that $\nu(p)+\nu(\overline p)<1$. Simply scaling them such that they sum up to one, \ie $\nu'(p)=\nicefrac{\nu(p)}{\nu(p)+\nu(\overline p)}$ and $\nu'(\overline p)=\nicefrac{\nu(\overline p)}{\nu(p)+\nu(\overline p)}$ induces a strictly smaller objective value. 

\nj{We can't explain this effect yet. I think we need a sellable argument in order to motivate why any iterative method on improving the objective value is needed.}

\paragraph{Possible Remedies.}
Adding scaling factors to the summands in the objective function helps improving the objective value:
\begin{align}
			\text{ minimize } &\quad \nicefrac{1}{p_{\sinit}} + \epsilon_1\cdot\sum_{p\in\Var}\frac{\epsilon_p}{p}\label{eq:min_geo_relax1}
\end{align}
for $\epsilon_1\in\R$ and $\epsilon_p\in\R$ for all $p\in\Var$. The factor $\epsilon$ favors maximizing the sum of parameters. This help to a certain extend getting stochastic solutions, \ie, satisfying Constraints~\ref{eq:well-defined_probs_geo} with equality. The individual factors $\epsilon_p$ for each parameter $p$ help in getting the probability $p_{\sinit}$ closer to the actual optimum.

Our experiments with the example above indicated, that there is a minimal value for $\epsilon_1$ which still induces stochastic distributions and has the highest value for $p_{\sinit}$. Then, favoring certain parameters by increasing the $\epsilon_p$-values drives the solution even closer to the optimum. 

For the example, we have:
\begin{align}
			\text{ minimize } &\quad \nicefrac{1}{p_{0}} + \epsilon_1\cdot \nicefrac{\epsilon_p}{p} + \nicefrac{1}{\overline p}
\end{align}
for an $\epsilon_1$ that induces stochastic distributions and $\epsilon_p=1$. The corresponding assignment is called $\nu^*$ and we observe that $\nu^*(p)>\nu^*(\overline p)$ which means that $p$ is ``favored'' over $\overline p$. We take the value $\nu^*(p)$ and set $\epsilon_2=\nicefrac{\nu^*(p)}{1-\nu^*(p)}$ and reiterate this procedure. In general that means that we strengthen the favoring of certain parameters. In our example we were able to drive the solution closer to the optimum using this iterative heuristic. Note that at some point of the iteration, a smaller value for $\epsilon_1$ still induced stochastic distributions, indicating that a two stage iteration is possible here.


\section{Computing local maximum using geometric programming}

Note: This explanation is written for Case A and C. As the objective for Case B involves minimizing the probability, it is tricky to find a local maximum point for this case.

\lmc{I guees we need to figure out a way to compute the local maximum for case B.}

For case A, the NLP problem given by Equations~\ref{eq:min}-\ref{eq:well-defined_probs} is non-convex due to constraints in Equation~\ref{eq:well-defined_probs}. To find a local solution for these cases we compute the best local monomial approximation for the posynomial term in Equation~\ref{eq:well-defined_probs} near the initial guess $x(k)$ with following, where $x(k)$ is the vector that has the variable assignments from initial guess for previous iteration:

\begin{align*}
f(w)\approx f(x(k))\prod_{i=1}^{m}\Bigg(\dfrac{w_{i}}{x(k)_{i}}\Bigg)^{a\textsl{i}},
\end{align*}

\noindent where

\begin{align*}
a_{i}=\dfrac{x(k)_{i}}{f(x(k)}\dfrac{\partial f}{\partial x_{i}}
\end{align*}

which is evaluated at $x(k)$. The approximation would be valid for $w \approx x$ and the right-hand side is the best local monomial approximation of $f$ near $x$.

After computing $f(w)$, we solve the following problem:


		\begin{align}
			\text{maximize } &\quad p_{\sinit}\\
			\text{such that}\\
%							 &\quad p_{\sinit}\leq \lambda\label{eq:strategyah:lambda}\\
			\forall s\in T.	 &\quad p_s=1\\
			\forall s\in S\setminus T.	&\quad p_s = \sum_{s'\in S}	P(s,s')\cdot p_{s'}\\
			\forall s\in S.	 &\quad f(w_{s})=1\\
			&\quad (1/k)x(k)_{i}\leq x_{i} \leq kx(k)_{i}, i=1,2,...,n
		\end{align}
		
\noindent where $k > 1$ is the value that determines the trust region of the approximation, $f(w_{s})$ is the best local monomial approximation of $\sum_{s'\in S}P(s,s')$ in state $s$ and $n$ is the number of variables. Generally, we set $k \approx 1$ to make sure that the error of the approximation is small.

As this problem is a GP, we could solve this problem efficiently and the solution of this problem would be taken for the next iteration and we repeat this procedure until convergence to a local maximum. The procedure would be similar in Case C, as we would compute the local momomial approximation of the posynomials in Equations~\ref{eq:welldefined_sched_rand} and \ref{eq:well-defined_probs_rand}. Then, we would iteratively compute the next guess until we converge to a local maximum.



==> pics/macros.tex <==
%% Commands requiring trailing spaces
\DeclareMathOperator*{\argmin}{argmin} 

\newcommand{\ie}{i.e.\@\xspace}
\newcommand{\wrt}{w.r.t.\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
\newcommand{\cf}{cf.\@\xspace}
\newcommand{\etal}{\emph{et al.}\@\xspace}
\newcommand{\prophesy}{\textrm{PROPhESY}\xspace}
\newcommand{\prism}{\textrm{PRISM}\xspace}
\newcommand{\storm}{\textrm{Storm}\xspace}
\newcommand{\tool}[1]{\textrm{#1}\xspace}


%%new commands
\newcommand{\dtmc}{\mathcal{D}}
\newcommand{\dtmcInit}[1][]{\ensuremath{\dtmc{#1}=(S{#1},\sinit{#1},P{#1})}}
\newcommand{\p}{\ensuremath{\mathbb{P}}}
\newcommand{\pr}{\ensuremath{\mathrm{Pr}}}
\newcommand{\reachPr}[2]{\ensuremath{\pr^{#1}(\finally #2)}}
\newcommand{\reachPrT}[1][]{\ensuremath{\reachPr{#1}{T}}}
\newcommand{\reachProp}[2]{\ensuremath{\p_{\leq #1}(\finally #2)}}
\newcommand{\reachProplT}{\ensuremath{\reachProp{\lambda}{T}}}
\newcommand{\reachPrs}[3]{\ensuremath{\pr^{#1}_{#2}(\finally #3)}}
%\newcommand{\reachPrsT}[2]{\ensuremath{\reachPrs{#1}{#2}{T}}}
\newcommand{\reachPropSymbol}{\varphi}
\newcommand{\ereachPropSymbol}{\psi}

\newcommand{\rew}{\ensuremath{r}}
\newcommand{\er}{\ensuremath{\mathrm{ER}}}
\newcommand{\expRew}[2]{\ensuremath{\er^{#1}(\finally #2)}}
\newcommand{\expRewT}[1][]{\ensuremath{\expRew{#1}{T}}}
\newcommand{\expRewProp}[2]{\ensuremath{\er_{\leq #1}(\finally #2)}}
\newcommand{\expRewPropkT}{\ensuremath{\expRewProp{\kappa}{T}}}
\newcommand{\rewFunction}{\ensuremath{\mathrm{rew}}}
\newcommand{\finally}{\lozenge}


\newcommand{\creachPr}[3]{\ensuremath{\pr^{#1}(\finally #2 \mathrel{|} \neg \finally #3)}}
\newcommand{\creachPrT}[1][]{\ensuremath{\creachPr{#1}{T}{U}}}
\newcommand{\creachProp}[3]{\ensuremath{\p_{\leq #1}(\finally #2 \mathrel{|} \neg \finally #3)}}
\newcommand{\creachProplT}{\ensuremath{\creachProp{\lambda}{T}{U}}}
\newcommand{\creachPrs}[4]{\ensuremath{\pr^{#1}_{#2}(\finally #3 \mathrel{|} #4)}}

\newcommand{\cexpRew}[3]{\ensuremath{\er^{#1}(\finally #2 \mathrel{|} \neg \finally #3)}}
\newcommand{\cexpRewT}[1][]{\ensuremath{\cexpRew{#1}{T}{U}}}

\newcommand{\cexpRewProp}[3]{\ensuremath{\rew_{\leq #1}(\finally #2 \mathrel{|} \neg \finally #3)}}
\newcommand{\cexpRewPropkT}{\ensuremath{\cexpRewProp{\kappa}{T}{U}}}



%% Comments
\newcommand{\commentside}[2]{\marginpar{\color{#1}\tiny#2}}
\newcommand{\TODO}[1]{\commentside{teal}{\textsc{Todo:} #1}}
\newcommand{\REMARK}[1]{\commentside{teal}{\textsc{Remark:} #1}}
\newcommand{\nj}[1]{\todo[inline,color=yellow!50]{\color{black}NJ: #1}\color{black}}
\newcommand{\lmc}[1]{\todo[inline,color=green!50]{\color{black}MC: #1}\color{black}}
%\newcommand{\njs}[1]{\commentside{yellow!70!black}{NJ: #1}}
\newcommand{\bk}[1]{\todo[inline,color=red!40]{BK: #1}}
%\newcommand{\bkss}[1]{\todo[color=red!40]{BK: #1}}
%\newcommand{\bks}[1]{\commentside{red!40}{BK: #1}}
\newcommand{\cd}[1]{\todo[inline,color=blue!40]{\color{black}CD: #1}\color{black}}
%\newcommand{\fos}[1]{\commentside{blue!40}{FO: #1}}
\newcommand{\lw}[1]{\todo[inline,color=green!70!black]{\color{black}LW: #1}\color{black}}
%\newcommand{\fgs}[1]{\commentside{green!70!black}{FG: #1}}
\newcommand{\jpk}[1]{\todo[inline,color=orange]{\color{white}JPK: #1}\color{black}}
%\newcommand{\jpks}[1]{\commentside{orange}{JPK: #1}}



%% Sets
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}

\newcommand{\Reals}{\ensuremath{\mathbb{R}}\xspace}    % Real numbers
\newcommand{\Rationals}{\ensuremath{\mathbb{Q}}\xspace}    %Rational numbers
\newcommand{\Integers}{\ensuremath{\mathbb{Z}}\xspace}    %Integer numbers
\newcommand{\Naturals}{\ensuremath{\mathbb{N}}}
\newcommand{\Ireal}{[0,\, 1]\subseteq\mathbb{R}}  % real interval [0,1]
\newcommand{\Irat}{[0,\, 1]\subseteq\mathbb{Q}}  % rational interval [0,1]
\newcommand{\Ex}{\ensuremath{\mathbb{E}}\xspace}        % Expectations
\newcommand{\BEx}{\ensuremath{\mathbb{E}_{\scriptscriptstyle \leq 1}}\xspace}        % Expectations
\newcommand{\ExCPO}{\ensuremath{\mathcal{E}}\xspace}              % Cpo of unbounded expectations
\newcommand{\BExCPO}{\ensuremath{\mathcal{E}_{\leq 1}}\xspace}        % Cpo of bounded expectations
\newcommand{\EV}{\ensuremath{\mathbf{E}}}

\newcommand{\Distr}{\mathit{Distr}}
\newcommand{\subDistr}{\mathit{subDistr}}
\newcommand{\distDom}{X}
\newcommand{\distDomFin}{\DistDom=\{x_1,\, \ldots,\, x_n}
\newcommand{\distFunc}{\mu}
\newcommand{\distDomElem}{x}
\newcommand{\supp}{\mathit{supp}}
\newcommand{\bigland}{\ensuremath{\bigwedge}}
\newcommand{\biglor}{\ensuremath{\bigvee}}


%% Constants
\newcommand{\true}{\ensuremath{\mathsf{true}}\xspace}
\newcommand{\false}{\ensuremath{\mathsf{false}}\xspace}
\newcommand{\ExpZero}{\CteFun{0}\xspace}
\newcommand{\ExpOne}{\CteFun{1}\xspace}


%% Math operators
\newcommand{\dual}[1]{{#1}^{\mathcal{D}}\xspace}               % Dual 
\newcommand{\eqdef}{\triangleq}                              % Equality used for definitions
\DeclareMathOperator*{\lfp}{\boldsymbol \mu}            % Least fixed point
\DeclareMathOperator*{\gfp}{\boldsymbol \nu}            % Greatest fixed point
\newcommand{\suchthat}{\mydot}
\newcommand{\dom}{\ensuremath{\mathit{dom}}}

\newcommand{\mydot}{\ensuremath                         % Scope delimiter (eg forall, lambda abstractions)
  \raisebox{0pt}{${\scriptscriptstyle \bullet}~$}}
\newcommand{\CteFun}[1]{\ensuremath{\boldsymbol{#1}}\xspace}    % Constant function


%% Linear temporal logic
\newcommand{\Always}{\Box \, }
\newcommand{\Finally}{\lozenge \, }
\newcommand{\Ever}{\Diamond \, }
\newcommand{\Next}{\bigcirc \, }
\newcommand{\Until}{\mbox{$\, {\sf U}\,$}}
\newcommand{\Unless}{\mbox{$\, {\sf W}\,$}}


%% Program Semantics
\renewcommand{\wp}{{\sf wp}\xspace}
\newcommand{\wlp}{{\sf wlp}\xspace}
\newcommand{\wllp}{{\textsf{w}(\textsf{l})\textsf{p}}\xspace}
\newcommand{\cwp}{{\sf cwp}\xspace}
\newcommand{\cwlp}{{\sf cwlp}\xspace}
\newcommand{\cwllp}{{\textsf{cw}(\textsf{l})\textsf{p}}\xspace}
\newcommand{\qcwp}{\ensuremath{\mathsf{\ushortw{cw}p}}\xspace}
\newcommand{\qcwlp}{\ensuremath{\mathsf{\ushortw{cwl}p}}\xspace}
%\newcommand{\qcwllp}{\ensuremath{\mathsf{\ushortw{cw\textnormal{(}l\textnormal{)}}p}}\xspace}
\newcommand{\sem}[1]{\llbracket #1 \rrbracket}
\newcommand{\ToExp}[1]{\ensuremath{ \chi_{#1} }\xspace}    % Lifting of predicates into expectations
%\newcommand{\ToExp}[1]{\ensuremath{\left[ #1 \right]}\xspace}    % Lifting of predicat
 \newcommand{\Pre}{\Psi}
 \newcommand{\Post}{\Phi}
% \newcommand{\Inv}{\Theta}


%% pGCL LANGUAGE
\newcommand{\GCL}{\textnormal{\textsf{GCL}}\xspace}
\newcommand{\pGCL}{\textnormal{\textsf{pGCL}}\xspace}
\newcommand{\fpGCL}{\textnormal{$\textsf{pGCL}^{\boxtimes}$}\xspace}
\newcommand{\cpGCL}{\textnormal{\textsf{cpGCL}}\xspace}
\newcommand{\cfpGCL}{\textnormal{$\textsf{cpGCL}^{\boxtimes}$}\xspace}
%%% Set of variables,states,expressions,etc  
\newcommand{\Cmd}{\ensuremath{\mathcal{P}}\xspace}        % Set of programs
\newcommand{\Var}{\ensuremath{\mathcal{V}}\xspace}        % Set of program variables 
\newcommand{\Paramvar}{\ensuremath{{V}}\xspace}        % Set of program variables 

\newcommand{\RExpr}{\ensuremath{\mathcal{E}}\xspace}      % Set of arithmetical expressions   
\newcommand{\BExpr}{\ensuremath{\mathcal{B}}\xspace}      % Set of boolean expressions
\newcommand{\PDom}{\ensuremath{\mathfrak{P}}\xspace}
%\newcommand{\State}{\ensuremath{\mathbb{S}}\xspace}      
\newcommand{\Loop}{\textsf{loop}\xspace} % shorthand to talk about loops
\newcommand{\Body}{\textsf{body}\xspace}
\newcommand{\Init}{\textsf{init}\xspace}
\newcommand{\counter}{\textit{cntr}\xspace}
\newcommand{\intercepted}{\textit{int}\xspace}
\newcommand{\delivered}{\textit{del}\xspace}
\newcommand{\continue}{\textit{rerun}\xspace}
%%% Language constructs
\newcommand{\Skip}{{\tt skip}\xspace}
\newcommand{\Abort}{{\tt abort}\xspace}
\newcommand{\Ass}[2]{#1 \coloneqq #2}
\newcommand{\Observe}{\textnormal{\texttt{observe}}\xspace}
\newcommand{\PChoice}[3]{\{#1\} \, \left[#2 \right] \, \{#3\}}
\newcommand{\NDChoice}[2]{\{#1\} \, \Box \, \{#2\}}
\newcommand{\If}{{\tt if}\xspace}
\newcommand{\Then}{{\tt then}\xspace}
\newcommand{\Else}{{\tt else}\xspace}
\newcommand{\While}{{\tt while}\xspace}
\newcommand{\For}{{\tt while}\xspace}

\newcommand{\Do}{{\tt do}\xspace}
\newcommand{\Ite}{{\tt ite}\xspace}
\newcommand{\Cond}[3]{{\Ite} \, (#1) \allowbreak\, \{#2\} \allowbreak\, \{#3\}}
\newcommand{\WhileDo}[2]{{\While} \,\allowbreak (#1) \,\allowbreak \{#2\}}
\newcommand{\WhileDok}[3]{{\While}^{{}< #1} \,\allowbreak (#2) \,\allowbreak \{#3\}}
\newcommand{\Assert}{{\sf assert}\xspace}


%% Miscellania 
\newcommand{\Tr}{\ensuremath{\mathcal{T}}}    % Program transformation
\newcommand{\To}{\rightarrow}                          % Function space constructor
\newcommand{\subst}[2]{[#1 / #2]}
\newcommand{\ourunderscore}{\rule{1.5ex}{0.4pt}}


%% Operational Semantics
\newcommand{\sinit}{s_{\mathit{I}}} % initial state of DTMC/MDP
\newcommand{\mdp}{\mathcal{M}}
%\newcommand{\Mdp}[1][]{\ensuremath{\mdp{#1}=(S{#1},I{#1},\Act,\pmdp{#1})}}
\newcommand{\MdpInit}[1][]{\ensuremath{\mdp{#1}=(S{#1},\,\sinit{#1},\,\Act,\,\probmdp{#1})}}
\newcommand{\probmdp}{\mathcal{P}}
\newcommand{\functions}[1][]{\ensuremath{\mathbb{Q}_{#1}}}
\newcommand{\poly}[1][]{\ensuremath{\mathbb{Q}[#1]}}

%\newcommand{\rew}{\ensuremath{\mathbb{E}}}
%\newcommand{\er}{\ensuremath{\mathrm{ER}}}
%\newcommand{\expRew}[2]{\ensuremath{\er^{#1}(\finally #2)}}
%\newcommand{\expRewT}[1][]{\ensuremath{\expRew{#1}{T}}}
%\newcommand{\expRewProp}[2]{\ensuremath{\rew_{\leq #1}(\finally #2)}}
%\newcommand{\expRewPropkT}{\ensuremath{\expRewProp{\kappa}{T}}}
%\newcommand{\rewFunction}{\ensuremath{\mathrm{rew}}}


%\newcommand{\ratfunceval}{\ensuremath{\ratfunc[{V\setminus\dom(u)}]}}
%\newcommand{\evalratfunc}[2]{\ensuremath{#1[{#2}/u]}}
%\newcommand{\Rloop}{\ensuremath{R_{\mathit{loop}}}}
%\newcommand{\Rout}{\ensuremath{R_{\mathit{out}}}}
\newcommand{\pol}{\ensuremath{g}}
\newcommand{\Par}{\ensuremath{{V}}}
\newcommand{\Expr}{\ensuremath{\mathsf{Expr}}}
\newcommand{\rat}[1]{\ensuremath{\Rationals_{#1}}}
%\newcommand{\poly}[1]{\ensuremath{\Integers_{#1}}}
\newcommand{\rdtmc}{\ensuremath{\mathcal{R}}}
\newcommand{\Rdtmc}[3]{\ensuremath{\rdtmc_{#1}^{#2}\llbracket #3\rrbracket}}
\newcommand{\pdtmc}{\ensuremath{\mathcal{P}}}
\newcommand{\AP}{\ensuremath{\mathit{AP}}}
\renewcommand{\Pr}{\ensuremath{\textnormal{Pr}}}
\newcommand{\Prr}[1]{\ensuremath{\Pr^{#1}}}
\newcommand{\sched}{\ensuremath{\sigma}}
\newcommand{\Sched}{\ensuremath{\mathit{Sched}}}

\newcommand{\rmdp}{\ensuremath{\mathfrak{R}}}
\newcommand{\Rmdp}[3]{\ensuremath{\mdp_{#1}^{#2}\llbracket #3\rrbracket}}
\newcommand{\Act}{\ensuremath{\mathit{Act}}}
\newcommand{\act}{\ensuremath{\alpha}}
\newcommand{\pmdp}{\ensuremath{\mathcal{P}}}

\newcommand{\pathset}{\mathsf{Paths}}
\newcommand{\paths}[2]{\pathset(#1,\allowbreak\,#2)}
\newcommand{\pathsfin}{\pathset_{\mathit{fin}}}
\newcommand{\pathsinf}{\pathset_{\mathit{inf}}}
%\newcommand{\path}{\pi}
\newcommand{\fpath}{\hat\pi}
\newcommand{\last}[1]{\mathit{last}(#1)}
\newcommand{\bad}{\ensuremath{\lightning}}
\newcommand{\undesired}{\ensuremath{\langle \bad \rangle}\xspace}
\newcommand{\sinklabel}{\mathpzc{sink}\xspace}
\newcommand{\sink}{\ensuremath{\langle \sinklabel \rangle}\xspace}
%\newcommand{\expandable}{\ensuremath{\langle \mathpzc{expandable}\rangle}\xspace}

\newcommand{\term}{\ensuremath{{\downarrow}}}
\newcommand{\expandable}{\ensuremath{{\uparrow}}}
\newcommand{\exit}{\ensuremath{{\downarrow}}}
\newcommand{\ExpRew}[2]{\ensuremath{\textnormal{\textsf{ExpRew}}^{#1}\left(#2\right)}}
\newcommand{\LExpRew}[2]{\ensuremath{\textnormal{\textsf{LExpRew}}^{#1}\left(#2\right)}}
\newcommand{\CExpRew}[3]{\ensuremath{\textnormal{\textsf{CExpRew}}^{#1}\left(#2\,|\,#3\right)}}
\newcommand{\CLExpRew}[3]{\ensuremath{\textnormal{\textsf{CLExpRew}}^{#1}\left(#2\,|\,#3\right)}}
%temporary mdp stuff
\newcommand{\Rewset}{\mathfrak C}
\newcommand{\Paths}{\mbox{\sl Paths}}

%% Math-Fonts
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\def\presuper#1#2%
  {\mathop{}%
   \mathopen{\vphantom{#2}}^{#1}%
   \kern-\scriptspace%
   #2}
   
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=.5pt] (char) {#1};}}


==> pics/packages.tex <==
\usepackage{amsmath,amssymb,amsfonts}
\usepackage{mathtools}
%\usepackage{amsthm}
% \usepackage[pdfpagelabels=true,linktocpage]{hyperref}
\usepackage[usenames,dvipsnames]{color}
\usepackage{xcolor}
\usepackage{xspace}
\usepackage{microtype}
\usepackage{todonotes}
\usepackage{colonequals}
\usepackage{wasysym}
 \usepackage{booktabs}
\usepackage[affil-it]{authblk}



\usepackage{multirow}
\usepackage{multicol}

\usepackage{paralist}

\usepackage{subfigure}
\usepackage{url}
\usepackage{appendix}
\usepackage{graphicx}
\usepackage{float}
%\usepackage[pdfpagelabels=true]{hyperref}
\usepackage{algorithm}
\usepackage{listings}
%\usepackage{newalg}
\usepackage{nicefrac}
\usepackage{tikz} 
\usepackage{pgfplots}
%\usepgfplotslibrary{external}
%\pgfplotsset{compat=1.8}
%\tikzexternalize[prefix=TikzPictures/]
%\usepackage{marvosym}
\usepackage{wrapfig}




\lstset{
	basicstyle=\ttfamily,
    keywordstyle=\bfseries,
    showstringspaces=false,
    numbers=left,
    numberstyle=\tiny,
    morekeywords={}
}

\usetikzlibrary{arrows,decorations.pathmorphing,positioning,fit,trees,shapes,shadows,automata,calc} 
%\usetikzlibrary{patterns,arrows,arrows.meta,calc,shapes,shadows,decorations.pathmorphing,decorations.pathreplacing,automata,shapes.multipart,positioning,shapes.geometric,fit,circuits,trees,shapes.gates.logic.US,fit,automata,snakes,shapes.geometric}

\pagestyle{plain}

\tikzset{outline/.style args={#1}{%
  draw=#1,thick,fill=#1!50}}


==> pics/results_table.tex <==
\begin{tabular}[b]{@{}crrlrlrr@{}}
\toprule
Benchmark       & \#{}states & \#{}par     & specs      & \tool{MOSEK} (s)  & & Z3 \\
\midrule
BRP (pMC)   & $5382$   &  $2$    & $\er,\p,*$    & $23.17$ &($6.48$) & $-$                   \\
%	   & $28166$   &  $2$    & $\er,\p,*$    & $477.89$  &($73.88$) & $-$                  \\
   & $112646$   &  $2$    & $\er,\p,*$    & $3541.59$  &($463.74$) & $-$      \\
      & $112646$   &  $4$    & $\er,\p,*$    & $4173.33$  &($568.79$) & $-$              \\

  & $5382$   &  $2$    & $\er,\p$    & $3.61$   & &$904.11$                   \\
%  & $28166$   &  $2$    & $\er,\p$    & $52.105$  & &$\mathit{TO}$                  \\
  & $112646$   &  $2$    & $\er,\p$    & $479.08$  & &$\mathit{TO}$                  \\
  
NAND (pMC)  & $4122$   &  $2$    & $\er,\p,*$    & $14.67$ &($2.51$) & $-$                   \\
%  & $14322$   &  $2$    & $\er,\p,*$    & $80.92$ & ($13.91$) & $-$  \\
   & $35122$   &  $2$    & $\er,\p,*$    & $1182.41$ &($95.19$) & $-$                  \\
   & $4122$   &  $2$    & $\er,\p$    & $1.25$   && $1.14$                   \\
%   & $14322$   &  $2$    & $\er,\p$    & $9.81$  && $3.71$    \\
  & $35122$   &  $2$    & $\er,\p$    & $106.40$  && $11.49$                  \\
BRP (pMDP)   & $5466$   &  $2$    & $\er,\p,*$    & $31.04$ &($8.11$) & $-$                   \\      
%   & $28366$   &  $2$    & $\er,\p,*$    & $583.94$  &($72.91$) & $-$                   \\    
   & $112846$   &  $2$    & $\er,\p,*$    & $4319.16$  &($512.20$) & $-$                   \\    
   & $5466$   &  $2$    & $\er,\p$    & $4.93$  && $1174.20$                   \\      
%   & $28366$   &  $2$    & $\er,\p$    & $61.17$   && $\mathit{TO}$                   \\    
   & $112846$   &  $2$    & $\er,\p$    & $711.50$   && $\mathit{TO}$                   \\  
CONS (pMDP)  & $4112$   &  $2$    & $\er,\p,*$    & $102.93$  &($1.14$) & $-$                   \\      
%   & $16400$   &  $2$    & $\er,\p,*$    & $1474.73$  &($18.19$) & $-$                   \\    
   & $65552$   &  $2$    & $\er,\p,*$    & $\mathit{TO}$  &&  $-$                   \\    
   & $4112$   &  $2$    & $\er,\p$    & $6.13$   && $\mathit{TO}$                   \\      
%   & $16400$   &  $2$    & $\er,\p$    & $94.19$   && $\mathit{TO}$                   \\    
   & $65552$   &  $2$    & $\er,\p$    & $1361.96$  & & $\mathit{TO}$                   \\  
\bottomrule\end{tabular}

